Proceedings of SuperB Workshop VI: New Physics at the Super Flavor Factory

The sixth SuperB Workshop was convened in response to questions posed by the INFN Review Committee, evaluating the SuperB project at the request of INFN. The working groups addressed the capability of a high-luminosity flavor factory that can gather a data sample of 50 to 75 /ab in five years to elucidate New Physics phenomena unearthed at the LHC. This report summarizes the results of the Workshop.

==> B-comp.tex <==
\section*{$B$ Physics}
%\section*{Comparison between Super$B$ and the KEKB upgrade}
\label{sec:B:UKEKB}

% {\bf  TIM IT IS FOR YOU... MARCO CAN ADD A PLOT IN SUSY FOR delta 1-3} \\

We must emphasise that the KEKB upgrade plan (to a peak
instantaneous luminosity of $2 \times 10^{35}$) cannot properly be called a Super
Flavor Factory. That title should be reserved for a collier that can accumulate
the data samples necessary for a precision study of flavor in the LHC era.
We expect that our colleagues who are the proponents of the KEKB upgrade, who
have for many years been promoting an upgrade to a higher luminosity, will
agree on this.

Secondly, we recall that a comparison must take into account not only the
available statistics (luminosity), but that the low backgrounds and improved
hermeticity (largely due to the smaller beam energy asymmetry) of \superb\
provide a significant enhancement for many analyses (especially recoil
analyses) that are crucial to the physics case of \superb.



\begin{table*}
  \begin{tabular}{|c|ccc|}
    \hline
    Mode & \multicolumn{3}{c|}{Sensitivity} \\
    & Current & Expected ($10 \ {\rm ab}^{-1}$) & Expected ($75 \ {\rm
      ab}^{-1}$)  \\
    \hline
    ${\cal B}(B \to X_s \gamma)$ & 7\% & 5\% & 3\% \\
    $A_{\CP}(B \to X_s \gamma)$ & 0.037 & 0.01 & 0.004--0.005 \\
    ${\cal B}(B^+ \to \tau^+ \nu)$ & 30\% & 10\% & 3--4\% \\
    ${\cal B}(B^+ \to \mu^+ \nu)$ & not measured & 20\% & 5--6\% \\
    ${\cal B}(B \to X_s l^+l^-)$ & 23\% & 15\% & 4--6\% \\
    $A_{{\rm FB}}(B \to X_s l^+l^-)_{s_0}$ & not measured & 30\% & 4--6\% \\
    ${\cal B}(B \to K \nu \overline{\nu})$ & not measured & not measured & 16--20\% \\
    $S(\KS \pi^0 \gamma)$ & 0.24 & 0.08 & 0.02--0.03 \\
    \hline
  \end{tabular}
  \caption{
    Comparison of current experimental sensitivities with those expected
    at the upgraded KEKB ($10 \ {\rm ab}^{-1}$)
    and at \superb\  ($75 \ {\rm  ab}^{-1}$).
    Only a small selection of observables are shown.
    Quoted sensitivities are relative uncertainties if given as a percentage,
    and absolute uncertainties otherwise.
    For more details, see text and Refs.~\cite{Bona:2007qt,Browder:2007gg,Browder:2008em}.
    \label{tab:ukekb-comp}
  }
\end{table*}

Due to the high power consumption, there is a question over how many months
per year KEKB can afford to run. However, we understand that the estimated
total integrated luminosity should be taken to be $10 \ {\rm ab}^{-1}$.  We do
not currently have an estimate of sensitivity with that data sample from the
KEKB upgrade proponents, and therefore we must rely on our own estimates.  We
also note that $2 \times 10^{35}$ is the maximum peak luminosity  specified for KEKB in the KEK Roadmap, whereas
$10^{36}$ is the baseline luminosity for \superb.

\begin{figure}[htb!]
    \label{fig:d13comp}
  \begin{center}
    \hspace{-0.7cm}\includegraphics[width=0.25\textwidth]{d13_ll_all_kek.eps}
    \hspace{-0.5cm}\includegraphics[width=0.25\textwidth]{d13_ll_all_superb.eps}
    \caption{
     Determination of the SUSY mass-insertion parameter $(\delta_{13})_{LL}$
     at the upgraded KEKB (left) and \superb\  (right).
    }
  \end{center}
\end{figure}


Table~\ref{tab:ukekb-comp} shows a quantitative comparison of the two
proposals.
This table contains only a small subset of the observables that will be
measured at \superb, including all the so-called ``golden processes'' of
Table~\ref{tab:golden}.
Here we make some additional comments on the entries of
Table~\ref{tab:ukekb-comp}

\begin{itemize}
\item
  The measurements of ${\cal B}(B \to X_s \gamma)$ and \hbox{${\cal B}(B^+ \to \ell^+ \nu)$ }
  are particularly important in the MFV scenarios described in
  Section~\ref{sec:B:pheno}.
  It is crucial to be able to search for small deviations from the SM value.
  Therefore the improvement is sensitivity provided by \superb is highly
  significant (see Figure~\ref{fig:btaunu}).
\item
The statistics of the upgraded KEKB is not sufficient to take advantage of
  the theoretical cleanliness of several inclusive observables, such as
  the zero-crossing of the forward-backward asymmetry in $b \to s\ell^+\ell^-$.
  Results with $10 \ {\rm ab}^{-1}$ would not match the precision from the
  exclusive mode $B \to K^* \mu^+\mu^-$, which will be measured by LHC$b$,
  but will be limited by hadronic uncertainties.
  \superb\  can provide a much more precise and theoretically clean measurement.
\item
  Several interesting rare decay modes, such as \hbox{$B \to K \nu \bar{\nu}$,}
  cannot be observed with the statistics of the upgraded KEKB
  (unless dramatic and unexpected New Physics enhancements are present).
  Preliminary studies are just starting on several other channels that fall
  into this category.  Examples are $B \to \gamma\gamma$ and $B \to$ invisible
  type decays, which are sensitive to New Physics models with extra-dimensions.
\item
  Another playground for comparison is the phenomenological analysis
  within the MSSM with generic mass insertion discussed in the CDR.
  Fig.~\ref{fig:d13comp} shows how well the $(\delta_{13})_{LL}$ can be
  reconstructed at \superb\  and with the KEKB upgrade. Lattice QCD
  performance, as discussed in the Appendix of the CDR, are assumed in both
  cases. The remarkable difference stems  mainly from the different performance
  in measuring the CKM parameters $\bar\rho$ and $\bar\eta$.

\end{itemize}



% The figure below shows a comparison of the exclusion plot in the
% $m(H^+)$--$\tan\beta$ plane coming from a measurement of ${\cal B}(B \to \tau
% \nu)$ with the different data samples (assuming that the result is consistent
% with the SM).  Note that this plot was specifically requested by the IRC
% during the meeting in November.  Another plot that will be prepared is the
% MSSM exclusion plot for various different luminosities (but with naive scaling
% of sensitivities).  A comparison of the sensitivities to NP at the (``worst
% case'') mSUGRA snowmass point (see below) may also be interesting.  However,
% we believe that a qualitative comparison of the physics reach may be more
% useful.

% The most obvious channel to demonstrate a dramatic improvement in the physics
% reach of Super$B$ compared to the KEKB upgrade is for lepton flavour violating
% $\tau$ decays ({\it e.g.} $\tau \to \mu \gamma$), but there are also several in
% $B$ physics.

% In the following we discuss very briefly few example of channels Super Flavour
% Factory luminosity are necessary  and could possibly be observed with data
% samples in excess of $10 \ {\rm ab}^{-1}$. Preliminary studies are just
% started.

% \begin{itemize}

% \item $B \to K \nu \bar{\nu}$ \\



% \item $B \to$ invisible \\
%   \indent in the SM, $B \to \nu \bar{\nu} \gamma$ has a branching fraction of
%   ${\cal O}(10^{-9})$ (${\cal B}(B \to \nu \bar{\nu})$ being negligibly
%   small); NP from {\it e.g.} models with extra-dimensions and light dark matter
%   permit ${\cal B}$ up to $10^{-5}$; the current limit is ${\cal O}(10^{-4})$
%   -- we will ask groups working on models with extra-dimensions to take look
%   at this channel

% \item $B \to l \nu$ \\


%   \indent discussed in the talks of A.~Bevan and S.~Robertson.  Note that $B
%   \to \mu \nu$ is experimentally cleaner and will eventually overtake $B \to
%   \tau \nu$ (which will become systematics limited) in terms of sensitivity to
%   small NP effects.  Furthermore, this channel allows a NP-sensitive
%   universality check from the ratio ${\cal B}(B \to \tau \nu)/{\cal B}(B \to
%   \mu \nu)$.

% \item ${\cal B}(b \to s \gamma)$ \\
%   \indent though this is likely systematics and/or theory limited

% \item ${\cal B}(b \to s l^+l^-)$ \\
%   \indent possibly theory limited

% \item zero crossing in the inclusive $b \to s l^+l^-$ forward-backward asymmetry

% \item we are also alert to other possibilities, including other rare channels
%   which are not necessarily discussed in the CDR.  We do not want to make an
%   excessively long list, but there are plenty of things to think about, {\it
%     e.g.} $B \to \gamma \gamma$, $B \to 4$leptons, ... Even $B_d \to \mu\mu$
%   could possibly be observed with data samples in excess of $100 \ {\rm
%     ab}^{-1}$.
% \end{itemize}

% % To conclude on this discussion, we recall that with a very high luminosity
% % Super Flavour Factory, such as Super$B$, there is a ``no lose theorem.''
% % For this to be the case, all observables must be measured as precisely as
% % possible.  We do not believe that this is true for the KEKB upgrade.


==> B-physics-UKEKB-comp.tex <==

\section*{Comparison between Super$B$ and the KEKB upgrade}
\label{sec:B:UKEKB}

% {\bf  TIM IT IS FOR YOU... MARCO CAN ADD A PLOT IN SUSY FOR delta 1-3} \\

First of all, we must emphasize that the KEKB upgrade plan (to a peak
instantaneous luminosity of $2 \times 10^{35}$) cannot be called a Super
Flavor Factory. That title must be reserved for a machine that can accumulate
the data samples necessary for a precision study of flavor in the LHC era.
We expect that our colleagues who are the proponents of the KEKB upgrade, who
have for many years been promoting an upgrade to a higher luminosity, will
agree on this.

Secondly, we recall that a comparison must take into account not only the
available statistics (luminosity), but that the low backgrounds and improved
hermeticity (largely due to the smaller beam energy asymmetry) of Super$B$
provide a significant enhancement for many analyses (especially recoil
analyses) that are crucial to the physics case of Super$B$.

Due to the high power consumption, there is a question over how many months
per year KEKB can afford to run. However, we understand that the estimated
total integrated luminosity should be taken to be $10 \ {\rm ab}^{-1}$.  We do
not currently have an estimate of sensitivity with that data sample from the
KEKB upgrade proponents, and therefore we must rely on our own estimates.  We
also note that $2 \times 10^{35}$ is a kind of maximum for KEKB, whereas
$10^{36}$ is a kind of baseline for Super$B$.

\begin{table*}[!htb]
  \begin{tabular}{|c|ccc|}
    \hline
    Mode & \multicolumn{3}{c|}{Sensitivity} \\
    & Current & Expected ($10 \ {\rm ab}^{-1}$) & Expected ($75 \ {\rm
      ab}^{-1}$)  \\
    \hline
    BR$(B \to X_s \gamma)$ & 7\% & 5\% & 3\% \\
    $A_{CP}(B \to X_s \gamma)$ & 0.037 & 0.01 & 0.004--0.005 \\
    BR$(B^+ \to \tau^+ \nu)$ & 30\% & 10\% & 3--4\% \\
    BR$(B^+ \to \mu^+ \nu)$ & not measured & 20\% & 5--6\% \\
    BR$(B \to X_s l^+l^-)$ & 23\% & 15\% & 4--6\% \\
    $A_{FB}(B \to X_s l^+l^-)_{s_0}$ & not measured & 30\% & 4--6\% \\
    BR$(B \to K \nu \overline{\nu})$ & not measured & not measured & 16--20\% \\
    $S(K_S \pi^0 \gamma)$ & 0.24 & 0.08 & 0.02--0.03 \\
    \hline
  \end{tabular}
  \caption{
    Comparison of current experimental sensitivities with those expected
    at the upgraded KEKB ($10 \ {\rm ab}^{-1}$)
    and at Super$B$ ($75 \ {\rm  ab}^{-1}$).
    Only a small selection of observables are shown.
    Quoted sensitivities are relative uncertainties if given as a percentage,
    and absolute uncertainties otherwise.
    For more details, see text and Refs.~\cite{Bona:2007qt,Browder:2007gg,Browder:2008em}.
    \label{tab:ukekb-comp}
  }
\end{table*}

Table~\ref{tab:ukekb-comp} shows a quantitative comparison of the two
proposals.
This table contains only a small subset of the observables that will be
measured at Super$B$, including all the so-called ``golden processes'' of
Table~\ref{tab:golden}.
Here we make some additional comments on the entries of
Table~\ref{tab:ukekb-comp}
\begin{itemize}
\item
  The measurements of BR$(B \to X_s \gamma)$ and BR$(B^+ \to \ell^+ \nu)$
  are particularly important in the MFV scenarios described in
  Section~\ref{sec:B:pheno}.
  It is crucial to be able to search for small deviations from the SM value.
  Therefore the improvement is sensitivity provided by Super$B$ is highly
  significant (see Figure~\ref{fig:btaunu}).
\item
  The statistics of the upgraded KEKB is not sufficient to take advantage of
  the theoretical cleanliness of several inclusive observables, such as
  the zero-crossing of the forward-backward asymmetry in $b \to s\ell^+\ell^-$.
  Results with $10 \ {\rm ab}^{-1}$ would not match the precision from the
  exclusive mode $B \to K^* \mu^+\mu^-$, which will be measured by LHCb,
  but will be limited by hadronic uncertainties.
  Super$B$ can provide a much more precise and theoretically clean measurement.
\item
  Several interesting rare decay modes, such as $B \to K \nu \bar{\nu}$,
  cannot be observed with the statistics of the upgraded KEKB
  (unless dramatic and unexpected NP enhancements are present).
  Preliminary studies are just starting on several other channels that fall
  into this category.  Examples are $B \to \gamma\gamma$ and $B \to$ invisible
  type decays, which are sensitive to NP models with extra-dimensions.
\item
  Another playground for comparison is the phenomenological analysis
  within the MSSM with generic mass insertion discussed in the CDR.
  Fig. ~\ref{fig:d13} shows how well the $(\delta_{13})_{LL}$ can be
  reconstructed at Super$B$ and with the KEK-$B$ upgrade. Lattice QCD
  performances as discussed in the Appendix of the CDR are assumed in both
  cases. The remarkable difference mainly stems from the different performances
  in measuring the CKM parameters $\bar\rho$ and $\bar\eta$.

\begin{figure}[!htb]
  \begin{center}
    \hspace{-0.7cm}\includegraphics[width=0.22\textwidth]{d13_ll_all_kek.eps}
    \hspace{-0.5cm}\includegraphics[width=0.22\textwidth]
{d13_ll_all_superb.eps}
    \caption{
     Determination of the SUSY mass-insertion parameter $(\delta_{13})_{LL}$
     at the upgraded KEKB (left) and SuperB (right).
    }
    \label{fig:d13}
  \end{center}
\end{figure}


\end{itemize}

% The figure below shows a comparison of the exclusion plot in the
% $m(H^+)$--$\tan\beta$ plane coming from a measurement of ${\cal B}(B \to \tau
% \nu)$ with the different data samples (assuming that the result is consistent
% with the SM).  Note that this plot was specifically requested by the IRC
% during the meeting in November.  Another plot that will be prepared is the
% MSSM exclusion plot for various different luminosities (but with naive scaling
% of sensitivities).  A comparison of the sensitivities to NP at the (``worst
% case'') mSUGRA snowmass point (see below) may also be interesting.  However,
% we believe that a qualitative comparison of the physics reach may be more
% useful.

% The most obvious channel to demonstrate a dramatic improvement in the physics
% reach of Super$B$ compared to the KEKB upgrade is for lepton flavor violating
% $\tau$ decays ({\it e.g.} $\tau \to \mu \gamma$), but there are also several in
% $B$ physics.

% In the following we discuss very briefly few example of channels Super Flavour
% Factory luminosity are necessary  and could possibly be observed with data
% samples in excess of $10 \ {\rm ab}^{-1}$. Preliminary studies are just
% started.

% \begin{itemize}

% \item $B \to K \nu \bar{\nu}$ \\



% \item $B \to$ invisible \\
%   \indent in the SM, $B \to \nu \bar{\nu} \gamma$ has a branching fraction of
%   ${\cal O}(10^{-9})$ (${\cal B}(B \to \nu \bar{\nu})$ being negligibly
%   small); NP from {\it e.g.} models with extra-dimensions and light dark matter
%   permit ${\cal B}$ up to $10^{-5}$; the current limit is ${\cal O}(10^{-4})$
%   -- we will ask groups working on models with extra-dimensions to take look
%   at this channel

% \item $B \to l \nu$ \\


%   \indent discussed in the talks of A.~Bevan and S.~Robertson.  Note that $B
%   \to \mu \nu$ is experimentally cleaner and will eventually overtake $B \to
%   \tau \nu$ (which will become systematics limited) in terms of sensitivity to
%   small NP effects.  Furthermore, this channel allows a NP-sensitive
%   universality check from the ratio ${\cal B}(B \to \tau \nu)/{\cal B}(B \to
%   \mu \nu)$.

% \item ${\cal B}(b \to s \gamma)$ \\
%   \indent though this is likely systematics and/or theory limited

% \item ${\cal B}(b \to s l^+l^-)$ \\
%   \indent possibly theory limited

% \item zero crossing in the inclusive $b \to s l^+l^-$ forward-backward asymmetry

% \item we are also alert to other possibilities, including other rare channels
%   which are not necessarily discussed in the CDR.  We do not want to make an
%   excessively long list, but there are plenty of things to think about, {\it
%     e.g.} $B \to \gamma \gamma$, $B \to 4$leptons, ... Even $B_d \to \mu\mu$
%   could possibly be observed with data samples in excess of $100 \ {\rm
%     ab}^{-1}$.
% \end{itemize}

% % To conclude on this discussion, we recall that with a very high luminosity
% % Super Flavour Factory, such as Super$B$, there is a ``no lose theorem.''
% % For this to be the case, all observables must be measured as precisely as
% % possible.  We do not believe that this is true for the KEKB upgrade.


==> B-physics-intro_org.tex <==
\section*{Introduction}
\label{sec:B:intro}

%In this note we summarise the activity of the working group on $B$ physics
%at the scientific retreat, ``SuperB Workshop VI: New Physics at the Super
%Flavour Factory \superb\,'' held January 7-15$^{\rm th}$, 2008 at IFIC in Valencia.
%
%Throughout the text we will attempt in a coherent manner to answer the
% questions we received  from the International Review Committee.

The physics case for \superb\ has been
discussed in some detail in the \superb\ Conceptual Design Report (henceforth CDR)~\cite{Bona:2007qt}.
In the CDR, and in the following, we consider the discovery potential of \superb\
in two scenarios: whether or not the LHC finds evidence for New Physics. \\

\noindent
{\bf LHC discovers new particles} \\
\par
\vskip - 9pt
\noindent
  If the LHC finds physics beyond the Standard Model, the essential, and unique, role of \superb\ will be to determine the flavor structure of the New Physics.  In that sense, measurements from \superb\ that
  are consistent with the Standard Model are as valuable as those that show
  significant deviations -- in either case these measurements provide information
  about the New Physics flavor structure that cannot be provided by other experiments.
%  In this context the goal then will no longer be to discover new physics,
%  but to measure its flavour properties.
  In this context, the measurement of  theoretically  clean rare  decays,
  even when found to be Standard Model-like, will yield valuable
  insights into the structure of New Physics models, providing
 information complementary to LHC results.

  It is, of course, generally regarded as more valuable to find deviations from Standard Model predictions than to
  find a result that agrees with the Standard Model, an, in fact,
  many New Physics flavor structures do produce measurable
  effects. As shown in the discussion on benchmark points below, there are also
  scenarios in which flavor effects can be very small, and perhaps barely visible, even
  with \superb. The great precision reached at \superb\ can still provide positive
  information on the underlying theory, even in a Standard Model-like flavor scenario.
  Indeed, we emphasize that measurement of the New Physics flavor couplings are the primary discovery goal of \superb;  results from both LHC and \superb\ are required to reconstruct the New Physics Lagrangian.\\

\noindent
{\bf There is no New Physics discovery at LHC} \\
\par
\vskip -9pt
\noindent
  If evidence for New Physics does not readily appear at LHC, the goal of \superb\ would
  then be emphasize measurement precision to search for deviations in
  flavor observables.  In this scenario, finding such small effects could provide the first
  evidence of New Physics!  The absence of knowledge about the New Physics scale from LHC would
  make it impossible to reconstruct the New Physics Lagrangian, but a New Physics discovery at
  \superb\ would provide a solid indication that the New Physics scale is only somewhat
  above the reach of LHC. \\

The chapter is organized as follows.
We first present a description of work done since
the writing of the CDR~\cite{Bona:2007qt}, concentrating on some particularly
interesting channels that were only partially covered or not covered at all.
IWe then update the phonomenological studies presented in the CDR,
including a classification of golden modes, perfomance at LHC benchmark points,
the impact of \superb\ on explicit models of SUSY breaking, and a brief discussion on
the interplay of flavor and high $p_{T}$ physics.
We concentrate on $B$ physics at the \FourS,
since we have little to add to  previous studies of
the potential for $B_s$ physics at the \FiveS~\cite{Baracchini:2007ei}.





















































==> B.tex <==
\part*{\centerline{$B$ Physics}}

\input{B-physics-intro}

\input{B-physics-channels}

\input{B-physics-pheno}

\input{B-physics-interplay}

\input{B-physics-UKEKB-comp}

\input{B-physics-bib}


==> Charm-comp-d.tex <==

\subsection*{Charm Physics}

The influence of New Physics on the charm sector is often overlooked. Flavor-changing neutral currents in the up quark sector are less suppressed than in the down quark sector. Thus high sensitivity studies of rare charm decays offer the possibility of isolating New Physics effects in $\DzDzb$ mixing, in \CP violation and in rare decay branching fractions.

The recent observation of substantial $\DzDzb$ mixing raises the very exciting possibility of measuring \CP violation in charm decays. Many of the most sensitive measurements remain statistics limited even with \superb\-size data samples, providing a substantial for gathering a sample many times that possible with the KEKB upgrade.

In several specific cases involving mixing, \CP violation in mixing can be studied more cleanly by taking advantage of the clean environment provided by exclusive $\DzDzb$ production at the $\psi(3770)$ resonance.  We have therefore included in the \superb\ design the capability of running at this center-of mass-energy. Long data-taking runs are not required; a run of two months duration at the $\pis(3770)$ would yield a data sample an order of magnitude larger than the total BES-III sample at that energy.

An upgraded KEKB is not capable of running at this reduced energy.




==> Tau-comp.tex <==

\subsection*{Tau Physics}

It is not unlikely that the most exciting results on New Physics in the flavor sector will be uncovered in $\tau$ decays.




==> aaa.tex <==
\relax 
\citation{GellMann:1964nj}
\citation{techni}
\citation{ibridi}
\citation{others}
\citation{mppr}
\citation{gell}
\citation{resu}
\citation{Caprini}
\citation{e791}
\citation{torni}
\citation{io}
\newlabel{FirstPage}{{}{1}{}{}{}}
\@writefile{toc}{\contentsline {section}{\numberline {I}Spectroscopy}{1}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {A} Light meson spectroscopy}{1}{}}
\citation{gribov}
\citation{jaffe}
\citation{wilc}
\citation{noim}
\citation{jaffe}
\citation{torni}
\citation{noim}
\citation{winprog}
\citation{winprog}
\citation{endnote1}
\newlabel{defdq}{{1}{2}{}{}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {1}{\ignorespaces Vector mesons ($q\mathaccent "7016\relax q$ states) and the sub-GeV scalar mesons in the $I_3-m$ plane.}}{2}{}}
\newlabel{i3}{{1}{2}{}{}{}}
\newlabel{exchange}{{2}{2}{}{}{}}
\newlabel{six}{{3}{2}{}{}{}}
\citation{winprog}
\citation{winprog}
\citation{winprog}
\citation{ginop}
\citation{Caprini}
\citation{ginop}
\citation{Caprini}
\citation{y2175}
\@writefile{lof}{\contentsline {figure}{\numberline {2}{\ignorespaces Decay of a tetraquark scalar meson $S$ in two $q \mathaccent "7016\relax {q}$ mesons $M_1 M_2$: (a) quark rearrangement (b) instanton-induced process.}}{3}{}}
\newlabel{qdiags}{{2}{3}{}{}{}}
\newlabel{einst}{{4}{3}{}{}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {3}{\ignorespaces Super-GeV scalar mesons in the $I_3-m$ plane.}}{3}{}}
\newlabel{i3h}{{3}{3}{}{}{}}
\@writefile{lot}{\contentsline {table}{\numberline {I}{\ignorespaces \relax \fontsize  {8}{9.5pt}\selectfont  \abovedisplayskip 6\p@ plus2\p@ minus4\p@ \belowdisplayskip \abovedisplayskip \abovedisplayshortskip \z@ plus\p@ \belowdisplayshortskip 3\p@ plus\p@ minus2\p@ \def \leftmargin \leftmargini \topsep 4\p@ plus2\p@ minus2\p@ \parsep 2\p@ plus\p@ minus\p@ \itemsep \parsep {\leftmargin \leftmargini \topsep 3\p@ plus\p@ minus\p@ \parsep 2\p@ plus\p@ minus\p@ \itemsep \parsep }Numerical results, amplitudes in GeV. Second and third columns: results obtained with a decay lagrangian including or not including instanton effects, respectively (Labels $I$ and no-$I$ mean that we do add or not the instanton contribution.). In this table no $f_0-\sigma $ mixing is assumed. Fourth column: best fit, see text, with instanton effects included. Fifth column: predictions for a $q\mathaccent "7016\relax q$ picture of the light scalars. The $\eta -\eta ^\prime $ singlet-octet mixing angle assumed: $\phi _{_{PS}}=-22^\circ $\nobreakspace  {}\cite  {ginop}. Data for $\sigma $ and $\kappa $ decays are from\nobreakspace  {}\cite  {Caprini}, the reported amplitudes correspond to: $\Gamma _{\rm  tot}(\sigma ) = 272 \pm 6$, $\Gamma _{\rm  tot}(\kappa ) = 557 \pm 24$. }}{3}{}}
\newlabel{tab:res}{{I}{3}{}{}{}}
\citation{Choi:2003ue}
\citation{Abulencia:2006ma}
\citation{Abe:2005iya}
\citation{babar:2007rv}
\citation{mppr}
\citation{Aubert:2005rm}
\citation{Aubert:2006ge}
\citation{belle:2007ea}
\citation{Aubert:2007pa}
\citation{belle:2007wg}
\citation{Maiani:2007vr}
\@writefile{toc}{\contentsline {subsection}{\numberline {B}Charmonium}{4}{}}
\newlabel{sec:data}{{I\,B}{4}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {C}\bf  {Bottomonium }}{4}{}}
\citation{Abe:2007tk}
\@writefile{lof}{\contentsline {figure}{\numberline {4}{\ignorespaces \it  Di-pion invariant mass distribution in $Y(4260)\ensuremath  {\rightarrow }\xspace  J/\psi \pi ^+\pi ^-$ (left), $Y(4350)\ensuremath  {\rightarrow }\xspace  \psi (2S) \pi ^+\pi ^-$ (center), and $Y(4660)\ensuremath  {\rightarrow }\xspace  \psi (2S) \pi ^+\pi ^-$ (right) decays. }}{5}{}}
\newlabel{fig:bellepipiinv}{{4}{5}{}{}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {5}{\ignorespaces \it  The $\psi (2S)\pi $ invariant mass distribution in $B\ensuremath  {\rightarrow }\xspace  \psi (2S)\pi K$ decays.}}{5}{}}
\newlabel{fig:belleZ4430}{{5}{5}{}{}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {6}{\ignorespaces \it  Measured masses of the newly observed states, positioned in the spectroscopy according to their most likely quantum numbers. The charged state ($Z(4430)$) has clearly no $C$ quantum number.}}{5}{}}
\newlabel{fig:summary}{{6}{5}{}{}{}}
\citation{Schael:2006cr}
\citation{Dermisek:2005gg}
\citation{Dermisek:2006py}
\citation{SanchisLozano:2007wv}
\citation{Gunion:2005rw}
\citation{McElrath:2005bp}
\citation{Fayet:2007ua}
\citation{Bird:2006jd}
\citation{Wilczek:1977zn}
\citation{Fullana:2007uq}
\citation{Dermisek:2005gg}
\citation{Domingo:2007dx}
\citation{Ellwanger:2005dv}
\citation{SanchisLozano:2008}
\citation{Ellwanger:2005dv}
\citation{SanchisLozano:2008}
\citation{SanchisLozano:2003ha}
\citation{SanchisLozano:2006gx}
\@writefile{toc}{\contentsline {subsection}{\numberline {D}Search for Physics Beyond the Standard Model in Bottomonium decays}{6}{}}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {1}Light Higgses}{6}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {7}{\ignorespaces Plot of $X_d=\mathop {\mathgroup \symoperators cos}\nolimits {\theta _A}$ $\mathop {\mathgroup \symoperators tan}\nolimits {\beta }$ (blue points) and $A_1$ mass in units of GeV (red crosses) versus $\mathop {\mathgroup \symoperators tan}\nolimits {\beta }$. All points were generated using the NMHDECAY code \cite  {Ellwanger:2005dv} satisfying both LEP and B-physics constraints using a particular set of NMSSM parameters \cite  {SanchisLozano:2008}.}}{6}{}}
\newlabel{ups_gamma_a_univers}{{I\,D\,1}{6}{}{}{}}
\citation{Ellwanger:2005dv}
\citation{Domingo:2007dx}
\citation{SanchisLozano:2007wv}
\citation{SanchisLozano:2008}
\citation{SanchisLozano:2003ha}
\citation{SanchisLozano:2006gx}
\citation{Fullana:2007uq}
\citation{McElrath:2005bp}
\citation{Gunion:2005rw}
\citation{endnote2}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {2}\bf  Invisible decays and light dark matter}{7}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {8}{\ignorespaces Plot of the $5 \sigma $ discover potential of a Super-B factory with $\Upsilon (3S)$ data, in the mode $\Upsilon (3S) \ensuremath  {\rightarrow }\xspace  \pi ^+ \pi ^- \Upsilon (1S) \ensuremath  {\rightarrow }\xspace  \pi ^+ \pi ^- \tau ^+ \tau ^- \gamma $ (solid black) and $\Upsilon (3S) \ensuremath  {\rightarrow }\xspace  \tau ^+ \tau ^- \gamma $ (dashed red). An integrated luminosity of 1 ab$^{-1}$ was assumed.}}{7}{}}
\newlabel{ups_gamma_a_mono}{{I\,D\,1}{7}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {E}Summary}{7}{}}
\bibcite{GellMann:1964nj}{{1}{}{{}}{{}}}
\bibcite{techni}{{2}{}{{}}{{}}}
\bibcite{ibridi}{{3}{}{{}}{{}}}
\bibcite{others}{{4}{}{{}}{{}}}
\bibcite{mppr}{{5}{}{{}}{{}}}
\bibcite{gell}{{6}{}{{}}{{}}}
\bibcite{resu}{{7}{}{{}}{{}}}
\bibcite{Caprini}{{8}{}{{}}{{}}}
\bibcite{e791}{{9}{}{{}}{{}}}
\bibcite{torni}{{10}{}{{}}{{}}}
\bibcite{io}{{11}{}{{}}{{}}}
\bibcite{gribov}{{12}{}{{}}{{}}}
\bibcite{jaffe}{{13}{}{{}}{{}}}
\bibcite{wilc}{{14}{}{{}}{{}}}
\bibcite{noim}{{15}{}{{}}{{}}}
\bibcite{winprog}{{16}{}{{}}{{}}}
\bibcite{ginop}{{17}{}{{}}{{}}}
\bibcite{y2175}{{18}{}{{}}{{}}}
\bibcite{Choi:2003ue}{{19}{}{{}}{{}}}
\bibcite{Abulencia:2006ma}{{20}{}{{}}{{}}}
\bibcite{Abe:2005iya}{{21}{}{{}}{{}}}
\bibcite{babar:2007rv}{{22}{}{{}}{{}}}
\bibcite{Aubert:2005rm}{{23}{}{{}}{{}}}
\bibcite{Aubert:2006ge}{{24}{}{{}}{{}}}
\bibcite{belle:2007ea}{{25}{}{{}}{{}}}
\bibcite{Aubert:2007pa}{{26}{}{{}}{{}}}
\bibcite{belle:2007wg}{{27}{}{{}}{{}}}
\bibcite{Maiani:2007vr}{{28}{}{{}}{{}}}
\bibcite{Abe:2007tk}{{29}{}{{}}{{}}}
\bibcite{Schael:2006cr}{{30}{}{{}}{{}}}
\bibcite{Dermisek:2005gg}{{31}{}{{}}{{}}}
\bibcite{Dermisek:2006py}{{32}{}{{}}{{}}}
\bibcite{SanchisLozano:2007wv}{{33}{}{{}}{{}}}
\bibcite{Fayet:2007ua}{{34}{}{{}}{{}}}
\bibcite{Bird:2006jd}{{35}{}{{}}{{}}}
\bibcite{McElrath:2005bp}{{36}{}{{}}{{}}}
\bibcite{Gunion:2005rw}{{37}{}{{}}{{}}}
\bibcite{Wilczek:1977zn}{{38}{}{{}}{{}}}
\bibcite{Fullana:2007uq}{{39}{}{{}}{{}}}
\bibcite{Domingo:2007dx}{{40}{}{{}}{{}}}
\@writefile{toc}{\contentsline {section}{\numberline {}References}{8}{}}
\bibcite{SanchisLozano:2003ha}{{41}{}{{}}{{}}}
\bibcite{SanchisLozano:2006gx}{{42}{}{{}}{{}}}
\bibcite{Ellwanger:2005dv}{{43}{}{{}}{{}}}
\bibcite{SanchisLozano:2008}{{44}{}{{}}{{}}}
\bibcite{endnote1}{{45}{}{{}}{{}}}
\bibcite{endnote2}{{46}{}{{}}{{}}}
\citation{Aubert:2006ge}
\global\NAT@numberstrue
\bibstyle{apsrev}
\newlabel{LastPage}{{}{8}}
\newlabel{LastBibItem}{{46}{9}{}{}{}}


==> babarsym.tex <==
%%%%%   Standard symbols for use in BABAR papers and BAD Notes
%%%%%
%%%%%   Revised   05/22/01 P. Dauncey     Added \hepex, etc. and clean up a bit
%%%%%   Revised   12/07/00 D. Hitlin      Added features of D. Kirkby's HEP.sty
%%%%%   Revised   07/13/00 R. Waldi       Corrected \Kbar, \Bbar ... macros
%%%%%   Revised   07/13/00 D. MacFarlane  Replaced incorrect \chic1 symbols
%%%%%   Revised   07/05/00 P. Dauncey     Added \mes, \mec, removed \O
%%%%%   Revised   07/04/00 D. MacFarlane  Added scalable version of BABAR
%%%%%   Revised   07/01/00 D. MacFarlane
%%%%%   Revised   06/21/00 D. Hitlin
%%%%%   Original  06/10/00 D. Hitlin
%%%%%   Revision of TDR and Physics Book symbol file
%%%%%

\RequirePackage{xspace}

%%%%%%%%%%%%%%%%%%%% BABAR ... THE NAME OF THE COLLABORATION %%%%

% Huge boldface
\def\hbabar{\mbox{{\huge\bf\sl B}\hspace{-0.1em}{\LARGE\bf\sl A}\hspace{-0.03em}{\huge\bf\sl B}\hspace{-0.1em}{\LARGE\bf\sl A\hspace{-0.03em}R}}}
% LARGE
\def\Lbabar{\mbox{{\LARGE\sl B}\hspace{-0.15em}{\Large\sl A}\hspace{-0.07em}{\LARGE\sl B}\hspace{-0.15em}{\Large\sl A\hspace{-0.02em}R}}}
% Large
\def\lbabar{\mbox{{\large\sl B}\hspace{-0.4em} {\normalsize\sl A}\hspace{-0.03em}{\large\sl B}\hspace{-0.4em} {\normalsize\sl A\hspace{-0.02em}R}}}
% normal size
%\def\babar{\mbox{\sl B\hspace{-0.4em} {\small\sl A}\hspace{-0.37em} \sl B\hspace{-0.4em} {\small\sl A\hspace{-0.02em}R}}}
% replace normalsize with scalable version       dbm 7/4/00
\usepackage{relsize}
\def\babar{\mbox{\slshape B\kern-0.1em{\smaller A}\kern-0.1em
    B\kern-0.1em{\smaller A\kern-0.2em R}}}

\def\superb{Super\!\!\;$B$\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%   LEPTONS   %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\let\emi\en
\def\electron   {\ensuremath{e}\xspace}
\def\en         {\ensuremath{e^-}\xspace}   % electron negative (\em is taken)
\def\ep         {\ensuremath{e^+}\xspace}
\def\epm        {\ensuremath{e^\pm}\xspace}
\def\epem       {\ensuremath{e^+e^-}\xspace}
\def\ee         {\ensuremath{e^-e^-}\xspace}

\def\mmu        {\ensuremath{\mu}\xspace}
\def\mup        {\ensuremath{\mu^+}\xspace}
\def\mun        {\ensuremath{\mu^-}\xspace} % muon negative (\mum is taken)
\def\mumu       {\ensuremath{\mu^+\mu^-}\xspace}
\def\mtau       {\ensuremath{\tau}\xspace}

\def\taup       {\ensuremath{\tau^+}\xspace}
\def\taum       {\ensuremath{\tau^-}\xspace}
\def\tautau     {\ensuremath{\tau^+\tau^-}\xspace}

\def\ellm       {\ensuremath{\ell^-}\xspace}
\def\ellp       {\ensuremath{\ell^+}\xspace}
\def\ellell     {\ensuremath{\ell^+ \ell^-}\xspace}

\def\nub        {\ensuremath{\overline{\nu}}\xspace}
\def\nunub      {\ensuremath{\nu{\overline{\nu}}}\xspace}
\def\nub        {\ensuremath{\overline{\nu}}\xspace}
\def\nunub      {\ensuremath{\nu{\overline{\nu}}}\xspace}
\def\nue        {\ensuremath{\nu_e}\xspace}
\def\nueb       {\ensuremath{\nub_e}\xspace}
\def\nuenueb    {\ensuremath{\nue\nueb}\xspace}
\def\num        {\ensuremath{\nu_\mu}\xspace}
\def\numb       {\ensuremath{\nub_\mu}\xspace}
\def\numnumb    {\ensuremath{\num\numb}\xspace}
\def\nut        {\ensuremath{\nu_\tau}\xspace}
\def\nutb       {\ensuremath{\nub_\tau}\xspace}
\def\nutnutb    {\ensuremath{\nut\nutb}\xspace}
\def\nul        {\ensuremath{\nu_\ell}\xspace}
\def\nulb       {\ensuremath{\nub_\ell}\xspace}
\def\nulnulb    {\ensuremath{\nul\nulb}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%  PHOTONS  %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\g     {\ensuremath{\gamma}\xspace}
\def\gaga  {\ensuremath{\gamma\gamma}\xspace}  %% changed from \gg, which is >>
\def\ggstar{\ensuremath{\gamma\gamma^*}\xspace}

\def\ega    {\ensuremath{e\gamma}\xspace}
\def\game   {\ensuremath{\gamma e^-}\xspace}
\def\epemg  {\ensuremath{e^+e^-\gamma}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%  Other GAUGE BOSONS  %%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\H      {\ensuremath{H^0}\xspace}
\def\Hp     {\ensuremath{H^+}\xspace}
\def\Hm     {\ensuremath{H^-}\xspace}
\def\Hpm    {\ensuremath{H^\pm}\xspace}
\def\W      {\ensuremath{W}\xspace}
\def\Wp     {\ensuremath{W^+}\xspace}
\def\Wm     {\ensuremath{W^-}\xspace}
\def\Wpm    {\ensuremath{W^\pm}\xspace}
\def\Z      {\ensuremath{Z^0}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%   QUARKS   %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\q     {\ensuremath{q}\xspace}
\def\qbar  {\ensuremath{\overline q}\xspace}
\def\qqbar {\ensuremath{q\overline q}\xspace}
\def\u     {\ensuremath{u}\xspace}
\def\ubar  {\ensuremath{\overline u}\xspace}
\def\uubar {\ensuremath{u\overline u}\xspace}
\def\d     {\ensuremath{d}\xspace}
\def\dbar  {\ensuremath{\overline d}\xspace}
\def\ddbar {\ensuremath{d\overline d}\xspace}
\def\s     {\ensuremath{s}\xspace}
\def\sbar  {\ensuremath{\overline s}\xspace}
\def\ssbar {\ensuremath{s\overline s}\xspace}
\def\c     {\ensuremath{c}\xspace}
\def\cbar  {\ensuremath{\overline c}\xspace}
\def\ccbar {\ensuremath{c\overline c}\xspace}
\def\b     {\ensuremath{b}\xspace}
\def\bbar  {\ensuremath{\overline b}\xspace}
\def\bbbar {\ensuremath{b\overline b}\xspace}
\def\t     {\ensuremath{t}\xspace}
\def\tbar  {\ensuremath{\overline t}\xspace}
\def\tbar  {\ensuremath{\overline t}\xspace}
\def\ttbar {\ensuremath{t\overline t}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% LIGHT MESONS  %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\piz   {\ensuremath{\pi^0}\xspace}
\def\pizs  {\ensuremath{\pi^0\mbox\,\rm{s}}\xspace}
\def\ppz   {\ensuremath{\pi^0\pi^0}\xspace}
\def\pip   {\ensuremath{\pi^+}\xspace}
\def\pim   {\ensuremath{\pi^-}\xspace}
\def\pipi  {\ensuremath{\pi^+\pi^-}\xspace}
\def\pipm  {\ensuremath{\pi^\pm}\xspace}
\def\pimp  {\ensuremath{\pi^\mp}\xspace}

\def\kaon  {\ensuremath{K}\xspace}
%%% do NOT use ensuremath here
\def\Kbar  {\kern 0.2em\overline{\kern -0.2em K}{}\xspace}
\def\Kb    {\ensuremath{\Kbar}\xspace}
\def\Kz    {\ensuremath{K^0}\xspace}
\def\Kzb   {\ensuremath{\Kbar^0}\xspace}
\def\KzKzb {\ensuremath{\Kz \kern -0.16em \Kzb}\xspace}
\def\Kp    {\ensuremath{K^+}\xspace}
\def\Km    {\ensuremath{K^-}\xspace}
\def\Kpm   {\ensuremath{K^\pm}\xspace}
\def\Kmp   {\ensuremath{K^\mp}\xspace}
\def\KpKm  {\ensuremath{\Kp \kern -0.16em \Km}\xspace}
\def\KS    {\ensuremath{K^0_{\scriptscriptstyle S}}\xspace}
\def\KL    {\ensuremath{K^0_{\scriptscriptstyle L}}\xspace}
\def\Kstarz  {\ensuremath{K^{*0}}\xspace}
\def\Kstarzb {\ensuremath{\Kbar^{*0}}\xspace}
\def\Kstar   {\ensuremath{K^*}\xspace}
\def\Kstarb  {\ensuremath{\Kbar^*}\xspace}
\def\Kstarp  {\ensuremath{K^{*+}}\xspace}
\def\Kstarm  {\ensuremath{K^{*-}}\xspace}
\def\Kstarpm {\ensuremath{K^{*\pm}}\xspace}
\def\Kstarmp {\ensuremath{K^{*\mp}}\xspace}

\newcommand{\etapr}{\ensuremath{\eta^{\prime}}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% HEAVY MESONS  %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% do NOT use ensuremath here
\def\Dbar    {\kern 0.2em\overline{\kern -0.2em D}{}\xspace}
\def\Db      {\ensuremath{\Dbar}\xspace}
\def\Dz      {\ensuremath{D^0}\xspace}
\def\Dzb     {\ensuremath{\Dbar^0}\xspace}
\def\DzDzb   {\ensuremath{\Dz {\kern -0.16em \Dzb}}\xspace}
\def\Dp      {\ensuremath{D^+}\xspace}
\def\Dm      {\ensuremath{D^-}\xspace}
\def\Dpm     {\ensuremath{D^\pm}\xspace}
\def\Dmp     {\ensuremath{D^\mp}\xspace}
\def\DpDm    {\ensuremath{\Dp {\kern -0.16em \Dm}}\xspace}
\def\Dstar   {\ensuremath{D^*}\xspace}
\def\Dstarb  {\ensuremath{\Dbar^*}\xspace}
\def\Dstarz  {\ensuremath{D^{*0}}\xspace}
\def\Dstarzb {\ensuremath{\Dbar^{*0}}\xspace}
\def\Dstarp  {\ensuremath{D^{*+}}\xspace}
\def\Dstarm  {\ensuremath{D^{*-}}\xspace}
\def\Dstarpm {\ensuremath{D^{*\pm}}\xspace}
\def\Dstarmp {\ensuremath{D^{*\mp}}\xspace}
\def\Ds      {\ensuremath{D^+_s}\xspace}
\def\Dsb     {\ensuremath{\Dbar^+_s}\xspace}
\def\Dss     {\ensuremath{D^{*+}_s}\xspace}

% Obsolete
\newcommand{\dstr}{\ensuremath{\Dstar}\xspace}
\newcommand{\dstrstr}{\ensuremath{D^{**}}\xspace}
\newcommand{\dsp}{\ensuremath{\Dstarp}\xspace}
\newcommand{\dsm}{\ensuremath{\Dstarm}\xspace}
\newcommand{\dsz}{\ensuremath{\Dstarz}\xspace}


\def\B       {\ensuremath{B}\xspace}
%%% do NOT use ensuremath here
\def\Bbar    {\kern 0.18em\overline{\kern -0.18em B}{}\xspace}
\def\Bb      {\ensuremath{\Bbar}\xspace}
\def\BB      {\ensuremath{B\Bbar}\xspace}
\def\Bz      {\ensuremath{B^0}\xspace}
\def\Bzb     {\ensuremath{\Bbar^0}\xspace}
\def\BzBzb   {\ensuremath{\Bz {\kern -0.16em \Bzb}}\xspace}
\def\Bu      {\ensuremath{B^+}\xspace}
\def\Bub     {\ensuremath{B^-}\xspace}
\def\Bp      {\ensuremath{\Bu}\xspace}
\def\Bm      {\ensuremath{\Bub}\xspace}
\def\Bpm     {\ensuremath{B^\pm}\xspace}
\def\Bmp     {\ensuremath{B^\mp}\xspace}
\def\BpBm    {\ensuremath{\Bu {\kern -0.16em \Bub}}\xspace}
\def\Bs      {\ensuremath{B_s}\xspace}
\def\Bsb     {\ensuremath{\Bbar_s}\xspace}

% added by GHM on March 25, 2003 -- from Andrei Gritsan
\def\BorBbar    {\kern 0.18em\optbar{\kern -0.18em B}{}\xspace}
\def\DorDbar    {\kern 0.18em\optbar{\kern -0.18em D}{}\xspace}
\def\KorKbar    {\kern 0.18em\optbar{\kern -0.18em K}{}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%% ONIA %%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\jpsi     {\ensuremath{{J\mskip -3mu/\mskip -2mu\psi\mskip 2mu}}\xspace}
\def\psitwos  {\ensuremath{\psi{(2S)}}\xspace}
\def\psiprpr  {\ensuremath{\psi(3770)}\xspace}
\def\etac     {\ensuremath{\eta_c}\xspace}
\def\chiczero {\ensuremath{\chi_{c0}}\xspace}
\def\chicone  {\ensuremath{\chi_{c1}}\xspace}
\def\chictwo  {\ensuremath{\chi_{c2}}\xspace}
\mathchardef\Upsilon="7107
%\def\Y#1S{}% no space before {...}!
%\def\OneS  {\Y1S}
%\def\TwoS  {\Y2S}
%\def\ThreeS {\Y3S}
%\def\FourS {\Y4S}
%\def\FiveS {\Y5S}
\def\OneS {\ensuremath{\Upsilon{(1S)}}\xspace}
\def\TwoS {\ensuremath{\Upsilon{(2S)}}\xspace}
\def\ThreeS {\ensuremath{\Upsilon{(3S)}}\xspace}
\def\FourS {\ensuremath{\Upsilon{(4S)}}\xspace}
\def\FiveS {\ensuremath{\Upsilon{(5S)}}\xspace}
\def\NS {\ensuremath{\Upsilon{(nS)}}\xspace}

%\def\chic1{\ensuremath{\chi_{c1}}}
%\def\chic2{\ensuremath{\chi_{c2}}}
%\def\chic3{\ensuremath{\chi_{c3}}}
\def\chic#1{\ensuremath{\chi_{c#1}}\xspace} % dbm


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%% BARYONS %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\proton      {\ensuremath{p}\xspace}
\def\antiproton  {\ensuremath{\overline p}\xspace}
\def\neutron     {\ensuremath{n}\xspace}
\def\antineutron {\ensuremath{\overline n}\xspace}

\mathchardef\Deltares="7101
\mathchardef\Xi="7104
\mathchardef\Lambda="7103
\mathchardef\Sigma="7106
\mathchardef\Omega="710A

%%% do NOT use ensuremath here
\def\Deltabar{\kern 0.25em\overline{\kern -0.25em \Deltares}{}\xspace}
\def\Lbar{\kern 0.2em\overline{\kern -0.2em\Lambda\kern 0.05em}\kern-0.05em{}\xspace}
\def\Sigbar{\kern 0.2em\overline{\kern -0.2em \Sigma}{}\xspace}
\def\Xibar{\kern 0.2em\overline{\kern -0.2em \Xi}{}\xspace}
\def\Obar{\kern 0.2em\overline{\kern -0.2em \Omega}{}\xspace}
\def\Nbar{\kern 0.2em\overline{\kern -0.2em N}{}\xspace}
\def\Xb{\kern 0.2em\overline{\kern -0.2em X}{}\xspace}

\def\X {\ensuremath{X}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%% TAU BRANCHING FRACTIONS %%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\BR         {{\ensuremath{\cal B}\xspace}}
\def\BRtauptoe  {\ensuremath{\BR(\taup \to \ep)}\xspace}
\def\BRtaumtoe  {\ensuremath{\BR(\taum \to \en)}\xspace}
\def\BRtauptomu {\ensuremath{\BR(\taup \to \mup)}\xspace}
\def\BRtaumtomu {\ensuremath{\BR(\taum \to \mun)}\xspace}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%  LIGHT HADRON DECAYS %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\etaprepp}{\ensuremath{\etapr \to \eta \pipi}\xspace}
\newcommand{\etaprrg} {\ensuremath{\etapr \to \rho^0 \g}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%  B DECAYS   %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\bpsiks     {\ensuremath{\Bz \to \jpsi \KS}\xspace}
\def\bpsikst    {\ensuremath{\Bz \to \jpsi \Kstar}\xspace}
\def\bpsikl     {\ensuremath{\Bz \to \jpsi \KL}\xspace}
\def\bpsikzeropi{\ensuremath{\Bz \to \jpsi \Kstarz (\to \KL \piz)}\xspace}
\def\bpsikpluspi{\ensuremath{\Bu \to \jpsi \Kstarp (\to \KL \pip)}\xspace}
\def\bpsikpi    {\ensuremath{\Bz/\Bzb \to \jpsi (\to \mumu) \Kpm \pimp}\xspace}
\def\bupsik     {\ensuremath{\Bpm \to \jpsi (\to \mumu) \Kpm}\xspace}
\def\bpsiX      {\ensuremath{\Bz \to \jpsi \X}\xspace}

\def\Bzbtomu    {\ensuremath{\Bzb \to \mu \X}\xspace}
\def\Bzbtox     {\ensuremath{\Bzb \to \X}\xspace}
\def\Bztopipi   {\ensuremath{\Bz \to \pipi}\xspace}
\def\Bztokpi    {\ensuremath{\Bz \to \Kpm \pimp}\xspace}
\def\Bztorhopi  {\ensuremath{\Bz \to \rho^+ \pim}\xspace}
\def\Bztorhorho {\ensuremath{\Bz \to \rho \rho}\xspace}
\def\Bztokrho   {\ensuremath{\Bz \to K \rho}\xspace}
\def\Bztokstpi  {\ensuremath{\Bz \to \Kstar \pi}\xspace}
\def\Bztoapi    {\ensuremath{\Bz \to a_1 \pi}\xspace}
\def\Bztodd     {\ensuremath{\Bz \to \DpDm}\xspace}
\def\Bztodstd   {\ensuremath{\Bz \to \Dstarp \Dm}\xspace}
\def\Bztodstdst {\ensuremath{\Bz \to \Dstarp \Dstarm}\xspace}

\def\BtoDK      {\ensuremath{B \to DK}\xspace}
\def\Btodstlnu  {\ensuremath{B \to \Dstar \ell \nu}\xspace}
\def\Btodstdlnu {\ensuremath{B \to \Dstar(D) \ell \nu}\xspace}
\def\Btorholnu  {\ensuremath{B \to \rho \ell \nu}\xspace}
\def\Btopilnu   {\ensuremath{B \to \pi \ell \nu}\xspace}

\def\Btoetah    {\ensuremath{B \to \eta h}\xspace}
\def\Btoetaph   {\ensuremath{B \to \etapr h}\xspace}

\newcommand{\Betaprks}{\ensuremath{\Bz \to \etapr \KS}\xspace}
\newcommand{\Betaprkz}{\ensuremath{\Bz \to \etapr \Kz}\xspace}

\def\btosgam    {\ensuremath{b \to s \g}\xspace}
\def\btodgam    {\ensuremath{b \to d \g}\xspace}
\def\btosll     {\ensuremath{b \to s \ellell}\xspace}
\def\btosnunu   {\ensuremath{b \to s \nunub}\xspace}
\def\btosgaga   {\ensuremath{b \to s \gaga}\xspace}
\def\btosglue   {\ensuremath{b \to s g}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%  Y(4S) DECAYS   %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\upsbb   {\ensuremath{\FourS \to \BB}\xspace}
\def\upsbzbz {\ensuremath{\FourS \to \BzBzb}\xspace}
\def\upsbpbm {\ensuremath{\FourS \to \BpBm}\xspace}
\def\upspsikl{\ensuremath{\FourS \to (\bpsikl) (\Bzbtox)}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%  TAU DECAYS   %%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\tauptoe    {\ensuremath{\taup \to \ep \nunub}\xspace}
\def\taumtoe    {\ensuremath{\taum \to \en \nunub}\xspace}
\def\tauptomu   {\ensuremath{\taup \to \mup \nunub}\xspace}
\def\taumtomu   {\ensuremath{\taum \to \mun \nunub}\xspace}
\def\tauptopi   {\ensuremath{\taup \to \pip \nub}\xspace}
\def\taumtopi   {\ensuremath{\taum \to \pim \nu}\xspace}

\newcommand{\taumg}      {\ensuremath{\tau^{\pm} \to \mu^{\pm} \gamma}\xspace}
\newcommand{\taueg}      {\ensuremath{\tau^{\pm} \to e^{\pm} \gamma}\xspace}
\newcommand{\taulg}      {\ensuremath{\tau^{\pm} \to \ell^{\pm} \gamma}\xspace}
\newcommand{\taueee}      {\ensuremath{\tau^{\pm} \rightarrow e^{\pm}e^+e^-}\xspace }
\def\taummm      {\ensuremath{\tau^{\pm} \rightarrow \mu^{\pm}\mu^+\mu^-}\xspace }
\def\tauemm      {\ensuremath{\tau^{\pm} \rightarrow e^{\pm}\mu^+\mu^-}\xspace }
\def\taumee      {\ensuremath{\tau^{\pm} \rightarrow \mu^{\pm}e^+e^-}\xspace}
\def\taulh       {\ensuremath{\tau^{\pm} \rightarrow \ell^{\pm}h^0}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% GAMMA-GAMMA REACTIONS %%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\ggtopi     {\ensuremath{\gaga \to \pipi}\xspace}
\def\ggtopiz    {\ensuremath{\gaga \to \ppz}\xspace}
\def\ggstox     {\ensuremath{\ggstar \to \X(1420) \to \kaon \kaon \pi}\xspace}
\def\ggstoeta   {\ensuremath{\ggstar \to \eta(550) \to \pipi \piz}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%   KINEMATICS    %%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\ptot       {\mbox{$p$}\xspace}
%\def\pxy        {\mbox{$p_{\rm t}$}
\def\pxy        {\mbox{$p_T$}\xspace}
%\def\pt         {\mbox{$p_{\rm t}$}\xspace}
\def\pt         {\mbox{$p_T$}\xspace}
\def\mes        {\mbox{$m_{\rm ES}$}\xspace}
\def\mec        {\mbox{$m_{\rm EC}$}\xspace}
\def\DeltaE     {\mbox{$\Delta E$}\xspace}

\def\pbcm {\ensuremath{p^*_{\Bz}}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%   GEOMETRY    %%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\mphi       {\mbox{$\phi$}\xspace}
\def\mtheta     {\mbox{$\theta$}\xspace}
\def\ctheta     {\mbox{$\cos\theta$}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% ENERGY AND MOMENTUM %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\tev}{\ensuremath{\mathrm{\,Te\kern -0.1em V}}\xspace}
\newcommand{\gev}{\ensuremath{\mathrm{\,Ge\kern -0.1em V}}\xspace}
\newcommand{\mev}{\ensuremath{\mathrm{\,Me\kern -0.1em V}}\xspace}
\newcommand{\kev}{\ensuremath{\mathrm{\,ke\kern -0.1em V}}\xspace}
\newcommand{\ev}{\ensuremath{\mathrm{\,e\kern -0.1em V}}\xspace}
\newcommand{\gevc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V\!/}c}}\xspace}
\newcommand{\mevc}{\ensuremath{{\mathrm{\,Me\kern -0.1em V\!/}c}}\xspace}
\newcommand{\gevcc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V\!/}c^2}}\xspace}
\newcommand{\mevcc}{\ensuremath{{\mathrm{\,Me\kern -0.1em V\!/}c^2}}\xspace}
%\def\ev   {\ensuremath{\rm \,e\kern -0.08em V}}
%\def\kev  {\ensuremath{\rm \,ke\kern -0.08em V}}
%\def\mev  {\ensuremath{\rm \,Me\kern -0.08em V}}
%\def\gev  {\ensuremath{\rm \,Ge\kern -0.08em V}}
%\def\gevc {\ensuremath{\rm \,Ge\kern -0.08em V\!/c}}
%\def\gevc {\ensuremath{{\rm \,Ge\kern -0.08em V\!/}c}}
%\def\tev  {\ensuremath{\rm \,Te\kern -0.08em V}}
%\def\mevc {\ensuremath{\rm \,Me\kern -0.08em V\!/c}}
%\def\mevc {\ensuremath{{\rm \,Me\kern -0.08em V\!/}c}}
%\def\gevcc{\ensuremath{\rm \,Ge\kern -0.08em V\!/c^2}}
%\def\mevcc{\ensuremath{\rm \,Me\kern -0.08em V\!/c^2}}
%\def\gevcc{\ensuremath{{\rm \,Ge\kern -0.08em V\!/}c^2}}
%\def\mevcc{\ensuremath{{\rm \,Me\kern -0.08em V\!/}c^2}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% DISTANCE AND AREA %%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\syin {\ensuremath{^{\prime\prime}}\xspace}
\def\inch   {\ensuremath{\rm \,in}\xspace} % \in is taken
\def\ft   {\ensuremath{\rm \,ft}\xspace}
\def\km   {\ensuremath{{\rm \,km}}\xspace}
\def\m    {\ensuremath{{\rm \,m}}\xspace}
\def\cm   {\ensuremath{{\rm \,cm}}\xspace}
\def\cma  {\ensuremath{{\rm \,cm}^2}\xspace}
\def\mm   {\ensuremath{{\rm \,mm}}\xspace}
\def\mma  {\ensuremath{{\rm \,mm}^2}\xspace}
%\def\mum  {\ensuremath{{\rm \,\mum}}\xspace}
\def\mum  {\ensuremath{{\,\mu\rm m}}\xspace}%% mu meter
%\def\muma {\ensuremath{\rm \,\mum}^2\xspace}
\def\muma       {\ensuremath{{\,\mu\rm m}^2}\xspace}
\def\nm   {\ensuremath{{\rm \,nm}}\xspace}
\def\fm   {\ensuremath{{\rm \,fm}}\xspace}
\def\nm         {\ensuremath{{\rm \,nm}}\xspace}   %% nanometer
%
\def\barn{\ensuremath{{\rm \,b}}\xspace}
\def\barnhyph{\ensuremath{{\rm -b}}\xspace}
\def\mbarn{\ensuremath{{\rm \,mb}}\xspace}
\def\mbarnhyph{\ensuremath{{\rm -mb}}\xspace}
\def\nb         {\ensuremath{{\rm \,nb}}\xspace}
\def\invnb {\ensuremath{\mbox{\,nb}^{-1}}\xspace}
\def\pb {\ensuremath{{\rm \,pb}}\xspace}
\def\invpb {\ensuremath{\mbox{\,pb}^{-1}}\xspace}
\def\fb   {\ensuremath{\mbox{\,fb}}\xspace}
\def\invfb   {\ensuremath{\mbox{\,fb}^{-1}}\xspace}
\def\invab   {\ensuremath{\mbox{\,ab}^{-1}}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% TIME AND MASS  %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\mus  {\ensuremath{\rm \,\mus}\xspace}
\def\ns   {\ensuremath{\rm \,ns}\xspace}
\def\ps   {\ensuremath{\rm \,ps}\xspace}
\def\fs   {\ensuremath{\rm \,fs}\xspace}
\def\gm   {\ensuremath{\rm \,g}\xspace}

%%\def\s{\ensuremath{\rm {\,s}}} %% second - this displays nothing  - why?
\def\sec{\ensuremath{\rm {\,s}}\xspace}       %% second - this works - jw 4/19
\def\ms         {\ensuremath{{\rm \,ms}}\xspace}     %% millisecond
\def\mus        {\ensuremath{\,\mu{\rm s}}\xspace}    %% microsecond
\def\ns         {\ensuremath{{\rm \,ns}}\xspace}      %% nanosecond
\def\ps         {\ensuremath{{\rm \,ps}}\xspace}  %% picosecond


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%   MISCELLANEOUS %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\Xrad {\ensuremath{X_0}\xspace}
\def\NIL{\ensuremath{\lambda_{int}}\xspace}
\let\dgr\degrees


%\def\m          {\ensuremath{\rm \,m}}    %% meter
%\def\ma         {\ensuremath{\rm \,m}^2}  %% meter squared
%\def\cm         {\ensuremath{\rm \,cm}}   %% centimeter
%\def\cma        {\ensuremath{\rm \,cm}^2} %% centimeter squared
\def\cms         {\ensuremath{{\rm \,cm}^{-2} {\rm s}^{-1}}\xspace}
%\def\mm         {\ensuremath{\rm \,mm}}   %% millimeter
%\def\mma        {\ensuremath{\rm \,mm}^2} %% millimeter squared
%\def\mum        {\ensuremath{\,\mu\rm m}} %% mu meter
%\def\muma       {\ensuremath{\,\mu\rm m^2}}


\def\mic  {\ensuremath{\,\mu{\rm C}}\xspace}
\def\krad {\ensuremath{\rm \,krad}\xspace}
\def\cmc  {\ensuremath{{\rm \,cm}^3}\xspace}
\def\yr   {\ensuremath{\rm \,yr}\xspace}
\def\hr   {\ensuremath{\rm \,hr}\xspace}
\def\degc {\ensuremath{^\circ}{C}\xspace}
\def\degk {\ensuremath {\rm K}\xspace}
\def\degrees{\ensuremath{^{\circ}}\xspace}
\def\mrad{\ensuremath{\rm \,mrad}\xspace}               %% milliradian
\def\rad{\ensuremath{\rm \,rad}\xspace}
\def\mradhyph{\ensuremath{\rm -mr}\xspace}
%
\def\sx    {\ensuremath{\sigma_x}\xspace}
\def\sy    {\ensuremath{\sigma_y}\xspace}
\def\sz    {\ensuremath{\sigma_z}\xspace}

%\renewcommand{\bar}[1]{\overline{#1}}

% Some more (from Helen)
%\def\O{{\ensuremath{\cal O}}}  !!! This is a predefined LaTeX symbol !!!
\def\order{{\ensuremath{\cal O}}\xspace}
\def\L{{\ensuremath{\cal L}}\xspace}
\def\calL{{\ensuremath{\cal L}}\xspace}
%\def\S{{\ensuremath{\cal S}}}  !!! This is a predefined LaTeX symbol !!!
\def\calS{{\ensuremath{\cal S}}\xspace}
\def\calA{{\ensuremath{\cal A}}\xspace}
\def\calD{{\ensuremath{\cal D}}\xspace}
\def\calR{{\ensuremath{\cal R}}\xspace}

%% Arrows:
\def\ra                 {\ensuremath{\rightarrow}\xspace}
\def\to                 {\ensuremath{\rightarrow}\xspace}


\newcommand{\stat}{\ensuremath{\mathrm{(stat)}}\xspace}
\newcommand{\syst}{\ensuremath{\mathrm{(syst)}}\xspace}


\def\pep2{PEP-II}
\def\BF{$B$ Factory}
\def\abf {asymmetric \BF}
\def\sx    {\ensuremath{\sigma_x}\xspace}
\def\sy    {\ensuremath{\sigma_y}\xspace}
\def\sz    {\ensuremath{\sigma_z}\xspace}


\newcommand{\inverse}{\ensuremath{^{-1}}\xspace}
\newcommand{\dedx}{\ensuremath{\mathrm{d}\hspace{-0.1em}E/\mathrm{d}x}\xspace}
\newcommand{\chisq}{\ensuremath{\chi^2}\xspace}
\newcommand{\delm}{\ensuremath{m_{\dstr}-m_{\dz}}\xspace}
\newcommand{\lum} {\ensuremath{\mathcal{L}}\xspace}

\def\gsim{{~\raise.15em\hbox{$>$}\kern-.85em
          \lower.35em\hbox{$\sim$}~}\xspace}
\def\lsim{{~\raise.15em\hbox{$<$}\kern-.85em
          \lower.35em\hbox{$\sim$}~}\xspace}

\def\qsq                {\ensuremath{q^2}\xspace}


% Data processing
\def\kbytes     {\ensuremath{{\rm \,kbytes}}\xspace}
\def\kbsps      {\ensuremath{{\rm \,kbytes/s}}\xspace}
\def\kbits      {\ensuremath{{\rm \,kbits}}\xspace}
\def\kbsps      {\ensuremath{{\rm \,kbits/s}}\xspace}
\def\mbsps      {\ensuremath{{\rm \,Mbits/s}}\xspace}
\def\mbytes     {\ensuremath{{\rm \,Mbytes}}\xspace}
\def\mbps       {\ensuremath{{\rm \,Mbyte/s}}\xspace}
\def\mbsps      {\ensuremath{{\rm \,Mbytes/s}}\xspace}
\def\gbsps      {\ensuremath{{\rm \,Gbits/s}}\xspace}
\def\gbytes     {\ensuremath{{\rm \,Gbytes}}\xspace}
\def\gbsps      {\ensuremath{{\rm \,Gbytes/s}}\xspace}
\def\tbytes     {\ensuremath{{\rm \,Tbytes}}\xspace}
\def\tbpy       {\ensuremath{{\rm \,Tbytes/yr}}\xspace}
%




% QCD parameters

\newcommand{\as}{\ensuremath{\alpha_{\scriptscriptstyle S}}\xspace}
\newcommand{\MSb}{\ensuremath{\overline{\mathrm{MS}}}\xspace}
\newcommand{\LMSb}{%
  \ensuremath{\Lambda_{\overline{\scriptscriptstyle\mathrm{MS}}}}\xspace
}

% Electroweak parameters

\newcommand{\tw}{\ensuremath{\theta_{\scriptscriptstyle W}}\xspace}
\newcommand{\twb}{%
  \ensuremath{\overline{\theta}_{\scriptscriptstyle W}}\xspace
}
\newcommand{\Afb}[1]{{\ensuremath{A_{\scriptscriptstyle FB}^{#1}}}\xspace}
\newcommand{\gv}[1]{{\ensuremath{g_{\scriptscriptstyle V}^{#1}}}\xspace}
\newcommand{\ga}[1]{{\ensuremath{g_{\scriptscriptstyle A}^{#1}}}\xspace}
\newcommand{\gvb}[1]{{\ensuremath{\overline{g}_{\scriptscriptstyle V}^{#1}}}\xspace}
\newcommand{\gab}[1]{{\ensuremath{\overline{g}_{\scriptscriptstyle A}^{#1}}}\xspace}


% CKM, CP violation

\def\eps{\varepsilon\xspace}
\def\epsK{\varepsilon_K\xspace}
\def\epsB{\varepsilon_B\xspace}
\def\epsp{\varepsilon^\prime_K\xspace}

\def\CP                {\ensuremath{C\!P}\xspace}
%\def\CPT               {\ensuremath{C\!P\!T}\xspace}
\def\CPT               {\ensuremath{C\!PT}\xspace} % Looks better without \!
% added by GHM on March 25, 2003
\def\C       {\ensuremath{C}\xspace}
\def\P       {\ensuremath{P}\xspace}
\def\T       {\ensuremath{T}\xspace}



\def\epstag  {\ensuremath{\varepsilon_{\rm tag}}\xspace}
\def\tagfac  {\ensuremath{\epstag(1-2w)^2}\xspace}

\def\rhobar {\ensuremath{\overline \rho}\xspace}
\def\etabar {\ensuremath{\overline \eta}\xspace}
%\def\paramest {\ensuremath{{\hat A}, {\hat \rho}, {\hat \eta} }}
%\def\ssparamest {\ensuremath{{\hat A}, {\hat {\sin 2 \alpha}},
%{\hat {\sin 2 \beta}} }}
\def\meas {\ensuremath{|V_{cb}|, |\frac{V_{ub}}{V_{cb}}|,
|\varepsilon_K|, \Delta m_{B_d}}\xspace}

\def\Vud  {\ensuremath{|V_{ud}|}\xspace}
\def\Vcd  {\ensuremath{|V_{cd}|}\xspace}
\def\Vtd  {\ensuremath{|V_{td}|}\xspace}
\def\Vus  {\ensuremath{|V_{us}|}\xspace}
\def\Vcs  {\ensuremath{|V_{cs}|}\xspace}
\def\Vts  {\ensuremath{|V_{ts}|}\xspace}
\def\Vub  {\ensuremath{|V_{ub}|}\xspace}
\def\Vcb  {\ensuremath{|V_{cb}|}\xspace}
\def\Vtb  {\ensuremath{|V_{tb}|}\xspace}

%\def\sa{${\sin\! 2 \alpha  }$\xspace}
%\def\sb{${\sin\! 2 \beta   }$\xspace}
%\def\sg{${\sin\! 2 \gamma  }$\xspace}

% added by Gautier for tagging, tagmix, and sin2beta
\def\stwoa{\ensuremath{\sin\! 2 \alpha  }\xspace}
\def\stwob{\ensuremath{\sin\! 2 \beta   }\xspace}
\def\stwog{\ensuremath{\sin\! 2 \gamma  }\xspace}
\def\mistag{\ensuremath{w}\xspace}
\def\dilution{\ensuremath{\cal D}\xspace}
\def\deltaz{\ensuremath{{\rm \Delta}z}\xspace}
\def\deltat{\ensuremath{{\rm \Delta}t}\xspace}
\def\deltamd{\ensuremath{{\rm \Delta}m_d}\xspace}

\newcommand{\fsubd}{\ensuremath{f_D}}\xspace
\newcommand{\fds}{\ensuremath{f_{D_s}}\xspace}
\newcommand{\fsubb}{\ensuremath{f_B}\xspace}
\newcommand{\fbd}{\ensuremath{f_{B_d}}\xspace}
\newcommand{\fbs}{\ensuremath{f_{B_s}}\xspace}
\newcommand{\bsubb}{\ensuremath{B_B}\xspace}
\newcommand{\bbd}{\ensuremath{B_{B_d}}\xspace}
\newcommand{\bbs}{\ensuremath{B_{B_s}}\xspace}
\newcommand{\rgbb}{\ensuremath{\hat{B}_B}\xspace}
\newcommand{\rgbbd}{\ensuremath{\hat{B}_{B_d}}\xspace}
\newcommand{\rgbbs}{\ensuremath{\hat{B}_{B_s}}\xspace}
\newcommand{\rgbk}{\ensuremath{\hat{B}_K}\xspace}
\newcommand{\lqcd}{\ensuremath{\Lambda_{\mathrm{QCD}}}\xspace}

%\newcommand{\eqref}[1]{Eq.~(\ref{eq:#1})}
\newcommand{\secref}[1]{Section~\ref{sec:#1}}
\newcommand{\subsecref}[1]{Section~\ref{subsec:#1}}
\newcommand{\figref}[1]{Figure~\ref{fig:#1}}
\newcommand{\tabref}[1]{Table~\ref{tab:#1}}




% Journal References

% These bases are useful for ``submitted to'' when no volume is needed
\newcommand{\epjBase}        {Eur.\ Phys.\ Jour.\xspace}
\newcommand{\jprlBase}       {Phys.\ Rev.\ Lett.\xspace}
\newcommand{\jprBase}        {Phys.\ Rev.\xspace}
\newcommand{\jplBase}        {Phys.\ Lett.\xspace}
%\newcommand{\nimBaseA}       {Nucl.\ Instr.\ Meth.\xspace}
%\newcommand{\nimBaseB}       {Nucl.\ Instr.\ and Meth.\xspace}
%\newcommand{\nimBaseC}       {Nucl.\ Instr.\ and Methods\xspace}
%\newcommand{\nimBaseD}       {Nucl.\ Instrum.\ Methods\xspace}
%\newcommand{\nimBaseE}       {Nucl.\ Instrum.\ Meth.\xspace}
% update the following based on input from John Ripka, Asst. Editor at PRL, August 2006
\newcommand{\nimBaseA}       {Nucl.\ Instrum.\ Methods Phys.\ Res., Sect.\ A\xspace}
\newcommand{\nimBaseB}       {Nucl.\ Instrum.\ Methods Phys.\ Res., Sect.\ B\xspace}
\newcommand{\nimBaseC}       {Nucl.\ Instrum.\ Methods Phys.\ Res., Sect.\ C\xspace}
\newcommand{\nimBaseD}       {Nucl.\ Instrum.\ Methods Phys.\ Res., Sect.\ D\xspace}
\newcommand{\nimBaseE}       {Nucl.\ Instrum.\ Methods Phys.\ Res., Sect.\ E\xspace}
\newcommand{\npBase}         {Nucl.\ Phys.\xspace}
\newcommand{\zpBase}         {Z.\ Phys.\xspace}


\newcommand{\apas}      [1]  {{Acta Phys.\ Austr.\ Suppl.\ {\bf #1}}}
\newcommand{\app}       [1]  {{Acta Phys.\ Polon.\ {\bf #1}}}
\newcommand{\ace}       [1]  {{Adv.\ Cry.\ Eng.\ {\bf #1}}}
\newcommand{\anp}       [1]  {{Adv.\ Nucl.\ Phys.\ {\bf #1}}}
\newcommand{\annp}      [1]  {{Ann.\ Phys.\ {\bf #1}}}
\newcommand{\araa}      [1]  {{Ann.\ Rev.\ Astr.\ Ap.\ {\bf #1}}}
\newcommand{\arnps}     [1]  {{Ann.\ Rev.\ Nucl.\ Part.\ Sci.\ {\bf #1}}}
\newcommand{\arns}      [1]  {{Ann.\ Rev.\ Nucl.\ Sci.\ {\bf #1}}}
\newcommand{\appopt}    [1]  {{Appl.\ Opt.\ {\bf #1}}}
\newcommand{\japj}      [1]  {{Astro.\ Phys.\ J.\ {\bf #1}}}
\newcommand{\baps}      [1]  {{Bull.\ Am.\ Phys.\ Soc.\ {\bf #1}}}
\newcommand{\seis}      [1]  {{Bull.\ Seismological Soc.\ of Am.\ {\bf #1}}}
\newcommand{\cmp}       [1]  {{Commun.\ Math.\ Phys.\ {\bf #1}}}
\newcommand{\cnpp}      [1]  {{Comm.\ Nucl.\ Part.\ Phys.\ {\bf #1}}}
\newcommand{\cpc}       [1]  {{Comput.\ Phys.\ Commun.\ {\bf #1}}}
\newcommand{\epj}       [1]  {\epjBase\ {\bf #1}}
%\newcommand{\epjc}      [1]  {{Eur.\ Phys.\ Jour.\ C~{\bf #1}}}
\newcommand{\epjc}      [1]  {\epjBase\ C~{\bf #1}}
\newcommand{\fizika}    [1]  {{Fizika~{\bf #1}}}
\newcommand{\fp}        [1]  {{Fortschr.\ Phys.\ {\bf #1}}}
\newcommand{\ited}      [1]  {{IEEE Trans.\ Electron.\ Devices~{\bf #1}}}
\newcommand{\itns}      [1]  {{IEEE Trans.\ Nucl.\ Sci.\ {\bf #1}}}
\newcommand{\ijqe}      [1]  {{IEEE J.\ Quantum Electron.\ {\bf #1}}}
\newcommand{\ijmp}      [1]  {{Int.\ Jour.\ Mod.\ Phys.\ {\bf #1}}}
\newcommand{\ijmpa}     [1]  {{Int.\ J.\ Mod.\ Phys.\ {\bf A{\bf #1}}}}
\newcommand{\jl}        [1]  {{JETP Lett.\ {\bf #1}}}
\newcommand{\jetp}      [1]  {{JETP~{\bf #1}}}
\newcommand{\jpg}       [1]  {{J.\ Phys.\ {\bf G{\bf #1}}}}
\newcommand{\jap}       [1]  {{J.\ Appl.\ Phys.\ {\bf #1}}}
\newcommand{\jmp}       [1]  {{J.\ Math.\ Phys.\ {\bf #1}}}
\newcommand{\jmes}      [1]  {{J.\ Micro.\ Elec.\ Sys.\ {\bf #1}}}
%\newcommand{\josa}      [1]  {{J.\ Opt.\ Soc.\ Am.\ {\bf #1}}}
\newcommand{\mpl}       [1]  {{Mod.\ Phys.\ Lett.\ {\bf #1}}}

%\newcommand{\nim}       [1]  {{Nucl.\ Instrum.\ and Methods~{\bf #1}}}
\newcommand{\nim}       [1]  {\nimBaseC~{\bf #1}}
\newcommand{\nimaa}       [1]  {\nimBaseE~{\bf #1}}
%\newcommand{\nima}      [1]  {{Nucl.\ Instrum.\ Methods~{\bf A{\bf #1}}}}
\newcommand{\nima}      [1]  {\nimBaseA~{\bf #1}}
\newcommand{\nimb}      [1]  {\nimBaseB~{\bf #1}}
\newcommand{\nimc}      [1]  {\nimBaseC~{\bf #1}}
\newcommand{\nimd}      [1]  {\nimBaseD~{\bf #1}}
\newcommand{\nime}      [1]  {\nimBaseE~{\bf #1}}
% add commands for NIM articles from earlier periods
% for NIM articles from 1981-1983
\newcommand{\oldnim}    [1]  {Nucl.\ Instrum.\ Methods Phys.\ Res.~{\bf #1}}
% for NIM articles prior to 1981
\newcommand{\oldernim}  [1]  {Nucl.\ Instrum.\ Methods~{\bf #1}}

%\newcommand{\np}        [1]  {{Nucl.\ Phys.\ {\bf #1}}}
\newcommand{\np}        [1]  {\npBase\ {\bf #1}}
%\newcommand{\npb}       [1]  {{Nucl.\ Phys.\ {\bf B{\bf #1}}}}
\newcommand{\npb}       [1]  {\npBase\ B~{\bf #1}}
\newcommand{\npps}      [1]  {{Nucl.\ Phys.\ Proc.\ Suppl.\ {\bf #1}}}
\newcommand{\npaps}     [1]  {{Nucl.\ Phys.\ A~Proc.\ Suppl.\ {\bf #1}}}
\newcommand{\npbps}     [1]  {{Nucl.\ Phys.\ B~Proc.\ Suppl.\ {\bf #1}}}

\newcommand{\ncim}      [1]  {{Nuo.\ Cim.\ {\bf #1}}}
\newcommand{\optl}      [1]  {{Opt.\ Lett.\ {\bf #1}}}
\newcommand{\optcom}    [1]  {{Opt.\ Commun.\ {\bf #1}}}
\newcommand{\partacc}   [1]  {{Particle Acclerators~{\bf #1}}}
\newcommand{\pan}       [1]  {{Phys.\ Atom.\ Nuclei~{\bf #1}}}
\newcommand{\pflu}      [1]  {{Physics of Fluids~{\bf #1}}}
\newcommand{\ptoday}    [1]  {{Physics Today~{\bf #1}}}

%\newcommand{\jpl}       [1]  {{Phys.\ Lett.\ {\bf #1}}}      % dbm
\newcommand{\jpl}       [1]  {\jplBase\ {\bf #1}}
%\newcommand{\plb}       [1]  {{Phys.\ Lett.\ B~{\bf #1}}}   % dbm
\newcommand{\plb}       [1]  {\jplBase\ B~{\bf #1}}
\newcommand{\prep}      [1]  {{Phys.\ Rep.\ {\bf #1}}}
%\newcommand{\jprl}      [1]  {{Phys.\ Rev.\ Lett.\ {\bf #1}}} % dbm
\newcommand{\jprl}      [1]  {\jprlBase\ {\bf #1}}
%\newcommand{\pr}        [1]  {{Phys.\ Rev.\ {\bf #1}}}
\newcommand{\pr}        [1]  {\jprBase\ {\bf #1}}
%\newcommand{\jpra}      [1]  {{Phys.\ Rev.\ A~{\bf #1}}}
\newcommand{\jpra}      [1]  {\jprBase\ A~{\bf #1}}
%\newcommand{\jprd}      [1]  {{Phys.\ Rev.\ D~{\bf #1}}}
\newcommand{\jprd}      [1]  {\jprBase\ D~{\bf #1}}
%\newcommand{\jpre}      [1]  {{Phys.\ Rev.\ E~{\bf #1}}}
\newcommand{\jpre}      [1]  {\jprBase\ E~{\bf #1}}

\newcommand{\prsl}      [1]  {{Proc.\ Roy.\ Soc.\ Lond.\ {\bf #1}}}
\newcommand{\ppnp}      [1]  {{Prog.\ Part.\ Nucl.\ Phys.\ {\bf #1}}}
\newcommand{\progtp}    [1]  {{Prog.\ Theor.\ Phys.\ {\bf #1}}}
\newcommand{\rpp}       [1]  {{Rep.\ Prog.\ Phys.\ {\bf #1}}}
\newcommand{\jrmp}      [1]  {{Rev.\ Mod.\ Phys.\ {\bf #1}}}  % dbm
\newcommand{\rsi}       [1]  {{Rev.\ Sci.\ Instr.\ {\bf #1}}}
\newcommand{\sci}       [1]  {{Science~{\bf #1}}}
\newcommand{\sjnp}      [1]  {{Sov.\ J.\ Nucl.\ Phys.\ {\bf #1}}}
\newcommand{\spd}       [1]  {{Sov.\ Phys.\ Dokl.\ {\bf #1}}}
\newcommand{\spu}       [1]  {{Sov.\ Phys.\ Usp.\ {\bf #1}}}
\newcommand{\tmf}       [1]  {{Teor.\ Mat.\ Fiz.\ {\bf #1}}}
\newcommand{\yf}        [1]  {{Yad.\ Fiz.\ {\bf #1}}}
%\newcommand{\zp}        [1]  {{Z.\ Phys.\ {\bf #1}}}
\newcommand{\zp}        [1]  {\zpBase\ {\bf #1}}
%\newcommand{\zpc}       [1]  {{Z.\ Phys.\ C~{\bf #1}}}
\newcommand{\zpc}       [1]  {\zpBase\ C~{\bf #1}}
\newcommand{\zpr}       [1]  {{ZhETF Pis.\ Red.\ {\bf #1}}}

\newcommand{\hepex}     [1]  {hep-ex/{#1}}
\newcommand{\hepph}     [1]  {hep-ph/{#1}}
\newcommand{\hepth}     [1]  {hep-th/{#1}}


%%%%%%%%%%%%%%%%%%%% SOFTWARE PACKAGES %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\aslund     {\mbox{\tt Aslund}\xspace}
\def\bbsim      {\mbox{\tt BBsim}\xspace}
\def\beast      {\mbox{\tt Beast}\xspace}
\def\beget      {\mbox{\tt Beget}\xspace}
\def\Bta        {\mbox{\tt Beta}\xspace}
\def\betakfit   {\mbox{\tt BetaKfit}\xspace}
\def\cornelius  {\mbox{\tt Cornelius}\xspace}
\def\evtgen     {\mbox{\tt EvtGen}\xspace}
\def\euclid     {\mbox{\tt Euclid}\xspace}
\def\fitver     {\mbox{\tt FitVer}\xspace}
\def\fluka      {\mbox{\tt Fluka}\xspace}
\def\fortran    {\mbox{\tt Fortran}\xspace}
\def\gcalor     {\mbox{\tt GCalor}\xspace}
\def\geant      {\mbox{\tt GEANT}\xspace}
\def\gheisha    {\mbox{\tt Gheisha}\xspace}
\def\hemicosm   {\mbox{\tt HemiCosm}\xspace}
\def\hepevt     {\mbox{\tt{/HepEvt/}}\xspace}
\def\jetset74   {\mbox{\tt Jetset \hspace{-0.5em}7.\hspace{-0.2em}4}\xspace}
%\def\jetset     {\mbox{\tt Jetset \hspace{-0.5em}7.\hspace{-0.2em}4}}
\def\koralb     {\mbox{\tt KoralB}\xspace}
\def\minuit     {\mbox{\tt Minuit}\xspace}
\def\objegs     {\mbox{\tt Objegs}\xspace}
\def\paw        {\mbox{\tt Paw}\xspace}
\def\Root       {\mbox{\tt Root}\xspace}
\def\squaw      {\mbox{\tt Squaw}\xspace}
\def\stdhep     {\mbox{\tt StdHep}\xspace}
\def\trackerr   {\mbox{\tt TrackErr}\xspace}
\def\turtle     {\mbox{\tt Decay~Turtle}\xspace}


==> comp-bib.tex <==
\begin{thebibliography}{99}

\bibitem{Bona:2007qt}
  M.~Bona {\it et al.},
  %``SuperB: A High-Luminosity Asymmetric e+ e- Super Flavor Factory. Conceptual
  %Design Report,''
  arXiv:0709.0451 [hep-ex].
  %%CITATION = ARXIV:0709.0451;%%

%\cite{Browder:2007gg}
\bibitem{Browder:2007gg}
  T.~Browder, M.~Ciuchini, T.~Gershon, M.~Hazumi, T.~Hurth, Y.~Okada and A.~Stocchi,
  %``On the Physics Case of a Super Flavour Factory,''
  JHEP {\bf 0802} (2008) 110
  [arXiv:0710.3799 [hep-ph]].
  %%CITATION = JHEPA,0802,110;%%
%\cite{Browder:2008em}
\bibitem{Browder:2008em}
  T.~E.~Browder, T.~Gershon, D.~Pirjol, A.~Soni and J.~Zupan,
  %``New Physics at a Super Flavor Factory,''
  arXiv:0802.3201 [hep-ph].
  %%CITATION = ARXIV:0802.3201;%%

\end{thebibliography}


==> comp.tex <==
{\centerline{\rule[0in]{0.92\columnwidth}{2pt}}
\vspace {-0.7cm}
\part*{\centerline{\LARGE{\superb\ and SuperKEKB}}}
\vskip -8pt
{\centerline{\rule[ 0.15in]{0.92\columnwidth}{2pt}}

%\section*{\superb\ and SuperKEKB}

\input{Comparison/compintro}

\input{Comparison/B-comp}

\input{Comparison/Charm-comp}

\input{Comparison/Tau-comp}

\input{Comparison/Spectroscopy-comp}

\input{Comparison/comp-bib}

\bigskip

\onecolumngrid\twocolumngrid\hbox{}


==> compintro.tex <==

%\section{{Introduction}}

%\bigskip
\smallskip

We conclude with a brief comparison between the physics capabilities of \superb\ and SuperKEKB.  Any such comparison is perforce difficult, especially when provided by the proponents of one of the proposed projects. to  improve the precision of the comparison, let us list a few of the salient characteristics of the two collider projects as proposed

\begin{itemize}
\item \superb\ has an initial luminosity of \hbox{$10^{36}$ cm$^{-2}$s$^{-1}$}, and can therefore integrate 15 ab$^{-1}$ in a Snowmass Year of $10^7$ seconds. SuperKEKB, as embodied in the KEK Roadmap, will have a luminosity of $2\times 10^{35}$ cm$^{-2}$s$^{-1}$ and can thus integrate approximately 2 ab$^{-1}$ in the 200 days of running specified, assuming the same overall efficiency.
\item
\superb\ has a proposed upgrade path that can raise the peak luminosity to $2.5\times 10^{36}$ cm$^{-2}$s$^{-1}$. \hbox{SuperKEKB}  has the potential of reaching \hbox{$8 \times 10^{35}$ cm$^{-2}$s$^{-1}$} by 2027, but this is not included in the KEK Roadmap.
\item
The power consumption of \superb is 17 MW. The power consumption of SuperKEKB, which uses much higher beam currents to produce smaller luminosity, is much higher. We can find no documentation on the SuperKEKB  power consumption at $2\times 10^{35}$, but the consumption at $4 \times 10^{35}$ is quoted as 60 MW for RF alone.
\item
These higher currents produce very difficult detector backgrounds at SuperKEKB. As the currents at \superb\ are comparable to those at \pep2, backgrounds are a much less difficult issue. There are luminosity-associated backgrounds as well as current-associated backgrounds; these are currently under detailed study.
\item
It appears that $\tau$ physics will assume great importance as a probe of physics beyond the Standard Model. \superb\ includes in the baseline design an 85\% longitudinally polarized electron beam and spin rotators to facilitate the production of polarized $\tau$ pairs. This polarization is the key to the study of the structure of lepton-flavor-violating couplings in $\tau$ decay, as well as the search for a $\tau$ EDM, or for $\CP$ violation in $\tau$ decay. SuperKEKB cannot incorporate a polarized beam.
\item
The recent observation of large \DzDzb mixing raises the exciting prospect of finding $\CP$ violation in charm decay, which would almost certainly indicate physics beyond the Standard Model. \superb can attack this problem in a comprehensive manner, with high luminosity data sample in the \FourS region and at the $\psi(3770)$ resonance, as the collider is designed to run at lower center-of-mass energies, at reduced luminosity. With very short duration low energy runs, a data sample an order of magnitude greater than that of the final BESIII sample can readily be obtained. SuperKEKB cannot run at low energies.
\end{itemize}



==> extra_refs.tex <==
\end{document}

\bibitem{newX} 
G.~Gokhroo {\it et al.},
  %``Observation of a near-threshold D0 anti-D0 pi0 enhancement in B --> D0
  %anti-D0 pi0 K decay,''
  Phys.\ Rev.\ Lett.\  {\bf 97}, 162002 (2006)
  [arXiv:hep-ex/0606055];
  %%CITATION = PRLTA,97,162002;%%
   B.~Aubert {\it et al.}  [BABAR Collaboration],
  %``Study of Resonances in Exclusive B Decays to Dbar(*)D(*)K,''
  arXiv:0708.1565 [hep-ex].
  %%CITATION = ARXIV:0708.1565;%%

\bibitem{newZ}
K.~Abe {\it et al.}  [Belle Collaboration],
  %``Observation of a resonance-like structure in the pi^+- psi' mass
  %distribution in exclusive B-->K pi^+- psi' decays,''
  arXiv:0708.1790 [hep-ex];
  %%CITATION = ARXIV:0708.1790;%%
{\it Press Release:} http://www.kek.jp/intra-e/press/2007/BellePress11e.html

\bibitem{y4260}
B.~Aubert {\it et al.}  [BABAR Collaboration],
  %``Observation of a broad structure in the $\pi^+ \pi^- J/\psi$ mass spectrum
  %around 4.26-GeV/c$^2$,''
  Phys.\ Rev.\ Lett.\  {\bf 95}, 142001 (2005)
  [arXiv:hep-ex/0506081].
  %%CITATION = PRLTA,95,142001;%%

\bibitem{others2}
 E.~Braaten and M.~Kusunoki,
  %``Low-energy universality and the new charmonium resonance at 3870-MeV,''
  Phys.\ Rev.\  D {\bf 69}, 074005 (2004)
  [arXiv:hep-ph/0311147];
  %%CITATION = PHRVA,D69,074005;%%
F.~E.~Close and P.~R.~Page,
  %``The D*0 anti-D0 threshold resonance,''
  Phys.\ Lett.\  B {\bf 578}, 119 (2004)
  [arXiv:hep-ph/0309253];
  %%CITATION = PHLTA,B578,119;%%
N.~A.~Tornqvist,
  %``Isospin breaking of the narrow charmonium state of Belle at 3872-MeV as  a
  %deuson,''
  Phys.\ Lett.\  B {\bf 590}, 209 (2004)
  [arXiv:hep-ph/0402237];
  %%CITATION = PHLTA,B590,209;%%
E.~S.~Swanson,
  %``The new heavy mesons: A status report,''
  Phys.\ Rept.\  {\bf 429}, 243 (2006)
  [arXiv:hep-ph/0601110];
  %%CITATION = PRPLC,429,243;%%
  M.~B.~Voloshin,
  %``Molecular quarkonium,''
{\it In the Proceedings of 4th Flavor Physics and CP Violation Conference (FPCP 2006), Vancouver, British Columbia, Canada, 9-12 Apr 2006, pp
014}
  [arXiv:hep-ph/0605063];
  %%CITATION = ECONF,C060409,014;%%
 S.~Fleming, M.~Kusunoki, T.~Mehen and U.~van Kolck,
  %``Pion Interactions in the X(3872),''
  Phys.\ Rev.\  D {\bf 76}, 034006 (2007)
  [arXiv:hep-ph/0703168];
  %%CITATION = PHRVA,D76,034006;%%
E.~Braaten and M.~Lu,
  %``Line Shapes of the X(3872),''
  Phys.\ Rev.\  D {\bf 76}, 094028 (2007)
  [arXiv:0709.2697 [hep-ph]];
  %%CITATION = PHRVA,D76,094028;%%
 E.~Braaten and M.~Lu,
  %``The Effects of Charged Charm Mesons on the Line Shapes of the X(3872),''
  arXiv:0710.5482 [hep-ph];
  %%CITATION = ARXIV:0710.5482;%%
{\it As for other interpretations of the $Y(4260)$:} 
E.~Kou and O.~Pene,
  %``Suppressed decay into open charm for the Y(4260) being an hybrid,''
  Phys.\ Lett.\  B {\bf 631}, 164 (2005)
  [arXiv:hep-ph/0507119];
  %%CITATION = PHLTA,B631,164;%%
F.~E.~Close and P.~R.~Page,
  %``Gluonic charmonium resonances at BaBar and Belle?,''
  Phys.\ Lett.\  B {\bf 628}, 215 (2005)
  [arXiv:hep-ph/0507199].
  %%CITATION = PHLTA,B628,215;%%
{\it As for other interpretations of the $Z(4433)$:}
J.~L.~Rosner,
  %``Threshold effect and \pi^\pm \psi(2S) peak,''
  arXiv:0708.3496 [hep-ph];
  %%CITATION = ARXIV:0708.3496;%%
D.~V.~Bugg,
  %``Z+(4430) as a cusp in D*(2010)Dbar_1(2420),''
  arXiv:0709.1254 [hep-ph];
  %%CITATION = ARXIV:0709.1254;%%
S.~S.~Gershtein, A.~K.~Likhoded and G.~P.~Pronko,
  %``Possible nature of $Z^+(4430)$,''
  arXiv:0709.2058 [hep-ph];
  %%CITATION = ARXIV:0709.2058;%%
 G.~J.~Ding,
  %``Understanding the Charged Meson Z(4430),''
  arXiv:0711.1485 [hep-ph];
  %%CITATION = ARXIV:0711.1485;%%
X.~Liu, Y.~R.~Liu, W.~Z.~Deng and S.~L.~Zhu,
  %``Is Z^+(4430) a loosely bound molecular state?,''
  arXiv:0711.0494 [hep-ph];
  %%CITATION = ARXIV:0711.0494;%%
K.~m.~Cheung, W.~Y.~Keung and T.~C.~Yuan,
  %``Bottomed Analog of Z+(4433),''
  arXiv:0709.1312 [hep-ph];
  %%CITATION = ARXIV:0709.1312;%%
X.~Liu, Y.~R.~Liu, W.~Z.~Deng and S.~L.~Zhu,
  %``Is Z^+(4430) a loosely bound molecular state?,''
  arXiv:0711.0494 [hep-ph];
  %%CITATION = ARXIV:0711.0494;%%
  S.~H.~Lee, A.~Mihara, F.~S.~Navarra and M.~Nielsen,
  %``QCD sum rules study of the meson Z^+(4430),''
  arXiv:0710.1029 [hep-ph];
  %%CITATION = ARXIV:0710.1029;%%
 C.~Meng and K.~T.~Chao,
  %``$Z^+(4430)$ as a resonance in the $D_1(D_1^\prime)D^*$ channel,''
  arXiv:0708.4222 [hep-ph].
  %%CITATION = ARXIV:0708.4222;%%
  C.~F.~Qiao,
  %``A Uniform Description of the States Recently Observed at B-factories,''
  arXiv:0709.4066 [hep-ph].
  %%CITATION = ARXIV:0709.4066;%%
 
\bibitem{jaffe}
R.~L.~Jaffe,
  %``Multi-Quark Hadrons. 1. The Phenomenology Of (2 Quark 2 Anti-Quark)
  %Mesons,''
  Phys.\ Rev.\  D {\bf 15}, 267 (1977);
  %%CITATION = PHRVA,D15,267;%%
  Phys.\ Rev.\  D {\bf 15}, 281 (1977);
  %%CITATION = PHRVA,D15,281;%%
  Phys.\ Rept.\  {\bf 409}, 1 (2005)
  [Nucl.\ Phys.\ Proc.\ Suppl.\  {\bf 142}, 343 (2005)]
  [arXiv:hep-ph/0409065];
  %%CITATION = NUPHZ,142,343;%%
  R.~L.~Jaffe and F.~Wilczek,
  %``Diquarks and exotic spectroscopy,''
  Phys.\ Rev.\ Lett.\  {\bf 91}, 232003 (2003)
  [arXiv:hep-ph/0307341].
  %%CITATION = PRLTA,91,232003;%%


  
\bibitem{newlook}
L.~Maiani, F.~Piccinini, A.~D.~Polosa and V.~Riquer,
  %``A new look at scalar mesons,''
  Phys.\ Rev.\ Lett.\  {\bf 93}, 212002 (2004)
  [arXiv:hep-ph/0407017].
  %%CITATION = PRLTA,93,212002;%%
  
\bibitem{winprog}
{\it Work in Progress.}

\bibitem{y2175} 
 B.~Aubert {\it et al.}  [BABAR Collaboration],
  %``A structure at 2175-MeV in e+ e- --> Phi f0(980) observed via
  %initial-state radiation,''
  Phys.\ Rev.\  D {\bf 74}, 091103 (2006)
  [arXiv:hep-ex/0610018].
  %%CITATION = PHRVA,D74,091103;%%

\bibitem{newprl}
 L.~Maiani, A.~D.~Polosa and V.~Riquer,
  %``Indications of a Four-Quark Structure for the X(3872) and X(3876) Particles
  %from Recent Belle and BABAR Data,''
  Phys.\ Rev.\ Lett.\  {\bf 99}, 182003 (2007)
  [arXiv:0707.3354 [hep-ph]].
  %%CITATION = PRLTA,99,182003;%%

\bibitem{CR}
E.~Corrigan and P.~Ramond,
  %``A Note On The Quark Content Of Large Color Groups,''
  Phys.\ Lett.\  B {\bf 87}, 73 (1979);
  %%CITATION = PHLTA,B87,73;%%
{\it see also} 
F.~Sannino and J.~Schechter,
  %``Alternative Large Nc Schemes and Chiral Dynamics,''
  Phys.\ Rev.\  D {\bf 76}, 014014 (2007)
  [arXiv:0704.0602 [hep-ph]].
  %%CITATION = PHRVA,D76,014014;%%

%\bibitem{thooft}
%G.~'t Hooft,
  %``A PLANAR DIAGRAM THEORY FOR STRONG INTERACTIONS,''
%  Nucl.\ Phys.\  B {\bf 72}, 461 (1974).
  %%CITATION = NUPHA,B72,461;%%

\bibitem{raj}
K.~Rajagopal and F.~Wilczek,
  %``The condensed matter physics of QCD,''
  arXiv:hep-ph/0011333.
  %%CITATION = HEP-PH/0011333;%%

\bibitem{oth4q}
D.~Ebert, R.~N.~Faustov and V.~O.~Galkin,
  %``Masses of heavy tetraquarks in the relativistic quark model,''
  Phys.\ Lett.\  B {\bf 634}, 214 (2006)
  [arXiv:hep-ph/0512230];
  %%CITATION = PHLTA,B634,214;%%
K.~Terasaki,
  %``A new tetra-quark interpretation of X(3872),''
  arXiv:0706.3944 [hep-ph];
  %%CITATION = ARXIV:0706.3944;%%
 M.~V.~Carlucci, F.~Giannuzzi, G.~Nardulli, M.~Pellicoro and S.~Stramaglia,
  %``AdS-QCD quark-antiquark potential, meson spectrum and tetraquarks,''
  arXiv:0711.2014 [hep-ph].
  %%CITATION = ARXIV:0711.2014;%%







\end{thebibliography}


%\end{document}


==> spectroscopy.tex <==
\section{Heavy quarkonium spectroscopy}
The bound state of two heavy quarks has low enough energies that its 
spectroscopy is close to the non-relativistic interpretations of the 
atoms. The quantum numbers that are more appropriate to characterize a 
state are therefore, in decreasing order of energy splitting among 
different eigenstates, the radial excitation ($n$), the spatial angular 
momentum $L$, the spin $S$ and the total angular momentum $J$. Given 
this set of quantum numbers, the parity and charge conjugation of the 
states are derived by $P=(-1)^(L+1)$ and $C=(-1)^)L+S)$. 
Fig.~\ref{fig:quarkon} shows the mass and quantum number assignments of 
the 
well established charmonium and bottomonium states.
\begin{figure*}[!htb]
 \begin{tabular}{lr}
% \rotatebox{0}{
\epsfig{file=charmon_proceed.eps,height=6cm}%} 
&
% \rotatebox{0}{
\epsfig{file=bottom_proceed.eps,height=6cm}%}\\
\end{tabular}
 \caption{\it Charmonium (left) and Bottomonium (right) states with 
$L<=2$. The theory predictions are according to the potential models 
described in Ref.~\cite{Brambilla:2004wf}. 
 }
    \label{fig:quarkon}
\end{figure*}

\subsection{Charmonium spectroscopy}
Figure~\ref{fig:quarkon}a shows that all the predicted states below open charm
 threshold have been observed, leaving the search open only to states above the
 threshold. In this field the lastest developments concern the measurement of 
the paramaters and the quantum number assignment for the $J^{PC}=1^{--}$ 
states.

The BES collaboration has recently performed a fit to the $R$ scan 
results which takes into account interference between resonances more 
accurately~\cite{Ablikim:2007gd}. The updated parameters are reported in Tab.~\ref{tab:rscan}, compared with the most recent determinations.
 
\begin{table*}[!htb]
\begin{center} 
\caption{ 
Most recent determination of the  $J^{PC}=1^{--}$  charmonium states from BES~\cite{Ablikim:2007gd}, compared to the 2006 edition of the PDG~\cite{Yao:2006px} 
}
\label{tab:rscan} 

\begin{tabular}{|c|c|c|c|c|c|} \hline \hline
        &         &$\psi(3770)$  &$\psi(4040)$&$\psi(4160)$&$\psi(4415)$\\ \hline
$M$     &PDG2006  &3771.1$\pm$2.4&4039$\pm$1.0&4153$\pm$3  & 4421$\pm$4 \\
(MeV/$c^2$)          &BES '07 &3771.4$\pm$1.8& 4038.5$\pm$4.6 & 4191.6$\pm$6.0 & 4415.2$\pm$7.5\\\hline\hline
$\Gamma_{tot}$&PDG2006  &23.0$\pm$2.7&80$\pm$10    &103$\pm$8    &     62$\pm$20   \\
(MeV)         &BES '07      &25.4$\pm$6.5&81.2$\pm$14.4&72.7$\pm$15.1&73.3$\pm$21.2\\\hline\hline
\end{tabular} 
\end{center}
\end{table*}

The $J^{PC}=1^{--}$ assignment does not univocously identify the state, since both $^{2S+1}L_J=^3D_1$ and $^3D_1$ states would have it. The recent observation from Belle of the first exclusive decay of the $\psi(4415)\to DD^*_{2}(2460)$~\cite{belle:2007fq}, shows that this meson is predominantly $D$ wave. At the same time the study from CLEO-c of the $\psi(3770)\to\chi_{cJ}\gamma$~\cite{Briere:2006ff} confirms the dominance of the $D$ wave also in this meson. Both these assignments confirm the theoretical predictions as shown in Fig.~\ref{fig:quarkon}a.

\subsection{Bottomonium transitions}
Figure~\ref{fig:quarkon}b shows that the panorama in the bottomonium sector is
 much less complete, since there is a large number of states below the open bottom 
threshold which have not yet been observed. Moreover there is no recent announcement on the topic.

There are on the contrary plenty of results on the transitions between $J^{PC}=1^{--}$ states, i.e. between $Y(nS)$ 
and $Y(mS)$ states. These transitions are relevant because it is possible to predict both the 
di-pion invariant mass spectrum in the case of $Y(nS)\to Y(mS)\pi^+\pi^-$ decays, and the relative rate between these 
decays and the $Y(nS)\to Y(mS)\eta$ decays. These transitions allow therefore stringent tests of low energy QCD, in particular
of the predicitons of the Multipole Expansion~\cite{Kuang:2006me}. 

Recent measurements of the $Y(4S)\to Y(2S)\pi^+\pi^-$ decays from BaBar~\cite{Aubert:2006bm} showed a discrepancy with 
the above-mentioned predictions. Since such predictions mutuated the matrix elements from PCAC, CLEO-c recently published a 
comprehensive study of $Y(3S)\to Y(mS)\pi^+\pi^-$ decays under more general assumpions~\cite{cleo:2007sja}: a fit to the two distributions ($m=1,2$)
letting the matrix elements float shows a good agreement with the data, thus confirming the validity of the model. 


==> x.tex <==
\relax 
\@setckpt{/Spectroscopy/spectroscopy_superb}{
\setcounter{page}{1}
\setcounter{equation}{0}
\setcounter{enumi}{0}
\setcounter{enumii}{0}
\setcounter{enumiii}{0}
\setcounter{enumiv}{0}
\setcounter{footnote}{0}
\setcounter{mpfootnote}{0}
\setcounter{part}{0}
\setcounter{chapter}{0}
\setcounter{section}{0}
\setcounter{subsection}{0}
\setcounter{subsubsection}{0}
\setcounter{paragraph}{0}
\setcounter{subparagraph}{0}
\setcounter{figure}{0}
\setcounter{table}{0}
}

